Proceedings of the first workshop on Flavor Symmetries and consequences in Accelerators and Cosmology (FLASY2011)

The main goals of the first "Workshop on FLAvor SYmmetries and consequences in accelerators and cosmology" (FLASY) was to summarize the theoretical status of flavor symmetries, bringing together young researchers in the field to stimulate discussions and new collaborations, with the aim of investigating possible new physics scenarios to be tested at the LHC, as well as in future neutrino, cosmology experiments and dark matter searches.

==> Author/Author.tex <==
\begin{center}
{\bf Abstract}\\
\vskip5.mm
In my model.....
\end{center}

\vskip5.mm

\section{introduction}
Introduction

\section{model}
The model.....


\begin{center}
\begin{figure}[h!]
%\includegraphics[width=8cm]{Author/fig1.eps}
\end{figure}
\end{center}


\begin{thebibliography}{9}




\end{thebibliography}



==> Author/BenjaminKoch-old.tex <==
%Benjamin Koch$^{*a}$, Marco Aurelio D\'\i az$^{a}$, and Sebasti\'an Garc\'ia S\'aenz$^{a}$,

%$^{*}$ speaker

%$^a$ Pontificia Universidad Catolica Chile

%\begin{center}
{\bf Abstract}\\
%\vskip5.mm
We discuss the decays of
gravitinos in the model of partial split supersymmetry (PSS),
finding that for a large range of gravitino masses, the
two body decay channel is dominant.
Taking the gravitino as dark matter candidate 
and demanding that the model also describes the established
neutrino masses and mixings we show that one can derive
a theoretical upper limit for the gravitino mass within
this model. Finally we address questions that have been
raised during this workshop.
%\end{center}

\vskip5.mm

\section{introduction}
Split supersymmetry (SS) was originally proposed to address two of the most 
conspicuous 
problems of supersymmetric models, which are fast proton decay and excessive 
flavor changing neutral currents and CP violation \cite{ArkaniHamed:2004fb}. In
SS the 
solution to these problems is 
accomplished by considering all squarks and sleptons very massive, with a mass
scale 
$\widetilde m$ somewhere between the supersymmetric scale $M_{susy}$ and the
Grand 
Unification scale $M_{GUT}$. One of the Higgs bosons remains light, as usual in 
supersymmetric models, as well as the gauginos and higgsinos, with all these
particles 
having a mass accessible to the LHC \cite{Aad:2009wy}.
In addition to this,
the introduction of bilinear R-parity violation into this kind of
models allows for a rich phenomenology, especially in the neutrino sector
\cite{Barbier:2004ez,Nowakowski:1995dx,Hirsch:2000ef,Chun:2004mu,Diaz:2006ee,Diaz:2009yz,Sundrum:2009gv}.

A variation of this model is 
Partial Split Supersymmetry (PSS). In PSS all squarks and sleptons have a mass
of the order of
the SS mass scale $\widetilde m$, but both Higgs doublets remain with a mass at
the electroweak scale \cite{Diaz:2006ee,Sundrum:2009gv}. The addition of RpV to
this
model was introduced to be able to generate a solar neutrino 
mass \cite{Diaz:2006ee}. Loop contributions from neutral CP-even and CP-odd 
Higgs bosons are indeed able to do the job, producing not only the atmospheric
and solar masses, but also the atmospheric, solar, and reactor neutrino mixing 
angles \cite{Diaz:2009gf}.

In R-parity violating PSS the usual dark matter candidates
of supersymmetric models (the neutralinos) are unstable. 
However, the gravitino is an alternative to the neutralino.
Also the gravitino can decay into standard model particles,
but its decay is expected to be further suppressed by the
Planck mass $M_P$. This proceedings paper is essentially
a summary of \cite{Diaz:2011pc}.

\section{Partial Split Supersymmetry}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In PSS both Higgs doublets remain with a mass at the electroweak scale. As
it happens in SS, higgsinos, gauginos, and Higgs bosons interact via induced 
R-parity conserving couplings of the type,
%
\begin{eqnarray}
{\cal L}_{PSS}^{RpC} &\owns& 
-\textstyle{\frac{1}{\sqrt{2}}} H_u^\dagger
(\tilde g_u \sigma\widetilde W + \tilde g'_u\widetilde B)\widetilde H_u
-\textstyle{\frac{1}{\sqrt{2}}} H_d^\dagger
(\tilde g_d \sigma \widetilde W - \tilde g'_d \widetilde B)\widetilde H_d 
+\mathrm{h.c.},
\label{RpCterms}
\end{eqnarray}
%
where $\tilde g_u$, $\tilde g'_u$, $\tilde g_d$, and $\tilde g'_d$ are
couplings induced in the effective low energy lagrangian. At the SS scale
$\widetilde m$ they satisfy the boundary conditions,
%
$\tilde g_u=\tilde g_d=g\,,\qquad \tilde g'_u=\tilde g'_d=g'$,
evolving with independent RGE down to the electroweak scale. Similarly to the
MSSM, both Higgs fields acquire a vacuum expectation value $\langle H_u\rangle=v_u$
and $\langle H_d\rangle=v_d$, with the constraint 
$v^2=v_u^2+v_d^2=246\,{\mathrm{GeV}}^2$
and the definition $\tan\beta=v_u/v_d$. Gauginos and higgsinos mix forming the
neutralinos, with a mass matrix very similar to the one in the MSSM.
The relevant bi-linear R-parity violating couplings are
\begin{equation}
{\cal L}_{PSS}^{RpV} =
-\epsilon_i \widetilde H_u^T \epsilon L_i  
\ -\ 
\textstyle{\frac{1}{\sqrt{2}}} b_i H_u^T\epsilon
(\tilde g_d \sigma\widetilde W-\tilde g'_d\widetilde B)L_i 
\ + \ h.c., 
\label{LSS2HDMRpV}
\end{equation}
where the $b_i$ are the parameters of the lepton-higgs-gaugino interactions,
$\epsilon=i\sigma_2$, and the $\epsilon_i$ are the supersymmetric BRpV
parameters.
The effective neutrino mass matrix in this approach was found to be \cite{Diaz:2009gf}
%
\begin{equation}
{\bf M}_\nu|_{ij}=A\Lambda_i\Lambda_j+
C\epsilon_i\epsilon_j,
\quad  \mbox{with}\quad 
\Lambda_i=\mu b_i v_u+\epsilon_i v_d\quad,
\label{DpiH2HDM}
\end{equation}
%
where
%
\begin{equation}
A^{(0)}= \frac{M_1 \tilde g^2_d + M_2 \tilde g'^2_d}{4\det{M_{\chi^0}}}.
\label{A0}
\end{equation}
and where the coefficient $C$ arises from loop diagrams with virtual
mixed Higgs fields and neutralinos.
The theoretical background model will be further discussed in  a later section.
In order to make a connection with neutrino physics we will now turn
to the photino-neutrino mixing in this model $U_{\tilde \gamma \nu}$.
This mixing is governed by the same parameters as neutrino mass matrix.
Thus, imposing that the model fits neutrino data reduces the 
parameter space of PSS which translates into an allowed range for the
mixing $U_{\tilde \gamma \nu}$. The determination of this range
was done numerically. For example for $M_1=300\,$GeV one finds
\begin{equation}
2 \cdot 10^{-17}<U_{\tilde \gamma \nu}<3 \cdot 10^{-14}\quad.
\end{equation}
This range will be of importance in the context of gravitino decay.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Gravitino Decay and Induced Photon flux}

In R-parity violating models the gravitino can decay completely
into ordinary particles which should lead to an observable
signature from gravitino dark matter. In our calculations
of this signature we asume that$m_{3/2}<m_W$.

The first coupling that is relevant for gravitino decay is
\begin{equation} \label{coupleGravi}
{\cal L} \owns -\frac{1}{4M_P} \overline\psi_\mu \sigma^{\nu\rho}
\gamma^\mu \lambda_\gamma F_{\nu\rho}
\end{equation}
%
where $M_P$ is the Planck mass, $\psi_\mu$ is the spin-$3/2$ gravitino 
field, $\lambda_\gamma$ is the spin-$1/2$ photino field, 
$F_{\nu\rho}=\partial_\nu A_\rho-\partial_\rho A_\nu$ is the photon field
strength, and $A_\mu$ is the photon field.
This coupling gives rise to a vertex gravitino photon, photino.
Due to a violation of R-parity the photino can further transform into a 
neutrino. This tranforation is proportional to the mixingo between
photino and neutrino $U_{\tilde \gamma \nu}$.
The resulting two body decay rate is then
\begin{equation} \label{eq:2body}
\Gamma(\widetilde{G}\rightarrow\gamma\nu) = 
\frac{m_{3/2}^3}{32\pi M_P^2}|{U}_{\widetilde{\gamma}\nu}|^2.
\end{equation}
In PSS the mixing between photon and photino is
\begin{equation} \label{eq:gammamixing}
U_{\widetilde{\gamma}\nu_i}\simeq\frac{\mu}{2({\rm det}M_{\chi^0})} 
\left(\tilde{g}_dM_1s_W-\tilde{g}'_dM_2c_W\right)\Lambda_i.
\end{equation}
The constants here are parameters of PSS which are also relevant
for the generation of neutrino masses and mixings within this model.

In addition to this two body decay one has to take into account
also the possible three body decays.
When studying the three body decay a more general part
of the interaction Lagrangian comes into play
\bea\label{coupleGravi2}
{\mathcal{L}}&\owns&
-\frac{i}{\sqrt{2}M_P}\left[
(D^*_\mu\phi^{i*})\bar \psi_\nu \gamma^\mu \gamma^\nu P_L \chi^i-
(D_\mu \phi^i)\bar \chi^i P_R \gamma^\nu \gamma^\mu \psi_\nu
\right]\\ \nonumber
&&-\frac{i}{8 M_P}\bar \psi_\mu 
\left[ \gamma^\nu,\gamma^\rho\right]
\gamma^\mu \lambda^{(\alpha)a}F_{\nu \rho}^{(\alpha)a}\quad,
\eea
where the second line is in analogy to (\ref{coupleGravi}) and the first line
introduces additional couplings with scalar fields $\phi$.
The 3-body decays of the gravitino were studied in detail for the first time in 
\cite{Choi:2010jt,Choi:2010xn}, where explicit formulae are given. Nevertheless,
our calculations 
have yielded that the three-body results in \cite{Choi:2010jt} have to be
corrected.
We agree, however, with the conclusion that the 3-body decays are indeed
important, 
and cannot be neglected in general.
The interaction (\ref{coupleGravi2}) allows for various amplitdes that
contribute to the decay of a gravitino into a neutrino and two leptons with
opposite charge. The details of this calculation were given in
\cite{arXiv:1106.0308}. 
We find 3-body decay branching ratios for small gravitino
masses $m_{3/2}<20\,$GeV of the
order of $<15\%$.

If dark matter consists of those gravitinos, their
decays should contribute to the photon spectra observed 
by astrophysical experiments.
This contribution consists of a 
mono-energetic line of energy $m_{3/2}/2$ from the two-body decay, plus a 
continuum distribution from the three-body decays. The exact form of the 
spectrum, which depends on $m_{3/2}$ and $M_1$, was studied in detail in 
\cite{Choi:2010jt,Choi:2010xn} using an event generator. 
Since the first contribution is the dominant feature \cite{Buchmuller:2007ui}
only this will be considered.
Here we are interested
in obtaining constraints on the gravitino parameters, for which it suffices 
as an approximation to consider only the photon line from the two-body 
decay, as this is the most prominent feature of the spectrum for values 
of $M_1$ up to 1 TeV \cite{Choi:2010jt}.
Following established models of dark matter distribution
and photon flux propagation
\cite{Navarro:1995iw,Bertone:2007aw,Buchmuller:2007ui}
one obtains the diffenctial flux in dependence of the photon energy
due to (\ref{eq:2body}). This flux, which is supposed
to be strongly peaked at the gravitino mass, can be compared
to the photon flux from the same region of the sky, which was
measured by the Fermi LAT collaboration \cite{Abdo:2010nz}.
Since the observed flux does not show any strong peak,
this non-observation can be used to constrain the parameters 
of the decay rate (\ref{eq:2body}). This method is essentially analogous
to   \cite{Restrepo:2011rj,Huang:2011xr,GomezVargas:2011ph}.
One obtains
\begin{equation} \label{eq:constraint1}
\left(\frac{\tau_{3/2}}{10^{27}~{\rm s}}\right)>\frac{0.851}{p(m_{3/2})}
B(\widetilde{G}\rightarrow\gamma\nu) 
\left(\frac{m_{3/2}}{1~{\rm GeV}}\right)^{\gamma-2},
\end{equation}
where we parametrized the energy dependent resolution for the Fermi LAT
experiment
$\sigma=m_{3/2}p(m_{3/2})/2$ by
\begin{equation}
p(m_{3/2}) = 0.349-0.142\log\left(\frac{m_{3/2}}{2~
{\rm MeV}}\right)+0.019\log^2\left(\frac{m_{3/2}}{2~{\rm MeV}}\right).
\end{equation}
In equation (\ref{eq:constraint1}) further appears
the two body branching ratio of the gravitino decay $B$ and
the lifetime of the  gravitino $\tau_{3/2}$.

Now we are in place to combine the constraints from the neutrino
sector and from the observed photon spectrum.
Both constraints can be visualized in a $m_{3/2}-\tau_{3/2}$ plane as it is 
shown in figure \ref{fig1ben}.
\begin{center}
\begin{figure}[h!]
\includegraphics[width=8cm]{Author/r300p.pdf}
\caption{\it Allowed region for $M_1=300$ GeV}
\label{fig1ben}
\end{figure}
\end{center}
From this figure one can also read off the essential conclusion
of this study: PSS as a model for neutrino mass and the possibility
of gravitino dark matter leads to the prediction of an upper limit
of the gravitino mass in the range of $10\,$GeV.

\section{Questions and answers }
We would like use the remaining space to address some questions 
that were raised during the workshop. We appreciate those comments
because they lead to a better understanding of the basic mechanism
at work.
\begin{itemize}
\item {\it``A dimension five operator generating $\nu$-Majorana masses
needs to have (i) lepton number violation and (ii) it needs
to be proportional to the square of a $SU(2)_L$ breaking vacuum expectation value \cite{Weinberg:1979sa}. Are both conditions fulfilled?''}

Both conditions are fulfilled. Condition (i) is rather obvious due to the Majorana nature
of the term in the effective Lagrangian. The vacuum expectation value of condition (ii)
is somewhat hidden in the $C$-term of the equation \ref{DpiH2HDM} which
can be shown to be proportional to $m_Z^2$.
\item  {\it``In m-sugra a vanishing splitting between the real and imaginary s-neutrino
masses drives two of the three neutrino masses to zero. The same should
happen in this model where the s-neutrinos are integrated out''}

The splitting is controlled by the value of $\epsilon(i)B(i)\rightarrow B_{\epsilon}^i$
which in general does not necessarily have to be as small as in m-sugra.
Actually in PSS it is not small.
The reason for this to happen can be seen in equation (B7)
of the paper \cite{Diaz:2006ee}:
If one assumes very large s-neutrino masses $M_{Li}$
this tadpole equation demands equally large values of
$B_{\epsilon}^i \sim v_i M_{Li}^2/v_u$. Thus the mixing parameter
grows in such a way that the Higgses and the s-neutrinos
always mix. As it can be seen in equations (44,45) of the same
paper: The matching conditions between PSS and MSSM at the
large scale $\tilde{m}$ imply that this mixing has a definite value
$s_s^i\sim c_{\alpha}v_i/v_u$ .
There are also no problems from the side of the mass bounds
since the charged scalar/sbottom loops are suppressed by
the large mass scale of the sbottom. 

\item {\it There is a theorem in \cite{hep-ph/9701253} that states:
  If the real part and the imaginary part of the s-neutrino
have equal values $m_{sn Re}=m_{sn Im}$ then the
Majorana like B-L violating mass term has to vanish
which again implies neutrinos have to have zero mass $m_nu=0$. 
Is there a contradiction?}

No there is no contradiction.
The $m_H$ and the $m_A$ Higgses have a fixed
part of s-neutrino (as explained above), thus the general
statement of that paper predicts for the case of PSS: 
If $m_H=m_A$, then $m_\nu =0$;
That this statement is true can be seen from
\cite{Diaz:2009gf}:
Equations (12,13) of this paper show that
$m_H^2\approx m_A^2 +m_Z^2 sin^2(2 \beta)$,
thus the splitting is $\sim m_Z^2 sin^2(2 \beta)$.
However as one can see from equation (23) of the
same paper: If this splitting is zero, then also the
contribution to $m_\nu$ is zero.
This is the realization of the general statement in PSS. 

\item 
{\it It has been shown that: If there is no s-neutrino 
then there is no neutrino Majorana mass \cite{hep-ph/9701253}.
Is there a contradiction?}

No there is no contradiction.
Since the s-neutrinos mix with the Higgses due to
the possibly large parameter $B_\epsilon^i$ there is always
a part of the s-neutrino interaction eigenstates in PSS.
Thus, there is no contradiction with this theorem.
\end{itemize}

\begin{thebibliography}{9}
\bibitem{ArkaniHamed:2004fb}
  N.~Arkani-Hamed and S.~Dimopoulos,
  %``Supersymmetric unification without low energy supersymmetry and signatures
  %for fine-tuning at the LHC,''
  JHEP {\bf 0506}, 073 (2005)
  [arXiv:hep-th/0405159];
  %%CITATION = JHEPA,0506,073;%%
%\cite{Giudice:2004tc}
%\bibitem{Giudice:2004tc}
  G.~F.~Giudice and A.~Romanino,
  %``Split supersymmetry,''
  Nucl.\ Phys.\  B {\bf 699}, 65 (2004)
  [Erratum-ibid.\  B {\bf 706}, 65 (2005)]
  [arXiv:hep-ph/0406088].

\bibitem{Aad:2009wy}
  G.~Aad {\it et al.}  [The ATLAS Collaboration],
  %``Expected Performance of the ATLAS Experiment - Detector, Trigger and
  %Physics,''
  arXiv:0901.0512 [hep-ex].
  %%CITATION = ARXIV:0901.0512;%%

%\cite{Barbier:2004ez}
\bibitem{Barbier:2004ez}
  R.~Barbier {\it et al.},
  %``R-parity violating supersymmetry,''
  Phys.\ Rept.\  {\bf 420}, 1 (2005)
  [arXiv:hep-ph/0406039].
  %%CITATION = PRPLC,420,1;%%

%\cite{Nowakowski:1995dx}
\bibitem{Nowakowski:1995dx}
  M.~Nowakowski and A.~Pilaftsis,
  %``W and Z boson interactions in supersymmetric models with explicit R-parity
  %violation,''
  Nucl.\ Phys.\  B {\bf 461}, 19 (1996)
  [arXiv:hep-ph/9508271];
  %%CITATION = NUPHA,B461,19;%%
%\cite{Hempfling:1995wj}
%\bibitem{Hempfling:1995wj}
  R.~Hempfling,
  %``Neutrino Masses and Mixing Angles in SUSY-GUT Theories with explicit
  %R-Parity Breaking,''
  Nucl.\ Phys.\  B {\bf 478}, 3 (1996)
  [arXiv:hep-ph/9511288].
  %%CITATION = NUPHA,B478,3;%%

%\cite{Hirsch:2000ef}
\bibitem{Hirsch:2000ef}
  M.~Hirsch, M.~A.~Diaz, W.~Porod, J.~C.~Romao and J.~W.~F.~Valle,
  %``Neutrino masses and mixings from supersymmetry with bilinear R-parity
  %violation: A theory for solar and atmospheric neutrino oscillations,''
  Phys.\ Rev.\  D {\bf 62}, 113008 (2000)
  [Erratum-ibid.\  D {\bf 65}, 119901 (2002)]
  [arXiv:hep-ph/0004115].
  %%CITATION = PHRVA,D62,113008;%%

%\cite{Chun:2004mu}
\bibitem{Chun:2004mu}
  E.~J.~Chun and S.~C.~Park,
  %``Neutrino mass from R-parity violation in split supersymmetry,''
  JHEP {\bf 0501}, 009 (2005)
  [arXiv:hep-ph/0410242];
  %%CITATION = JHEPA,0501,009;%%
%\cite{Davidson:2000ne}
%\bibitem{Davidson:2000ne}
  S.~Davidson and M.~Losada,
  %``Basis independent neutrino masses in the R(p) violating MSSM,''
  Phys.\ Rev.\  D {\bf 65}, 075025 (2002)
  [arXiv:hep-ph/0010325];
  %%CITATION = PHRVA,D65,075025;%%
%\cite{Davidson:2000uc}
%\bibitem{Davidson:2000uc}
  S.~Davidson and M.~Losada,
  %``Neutrino masses in the R(p) violating MSSM,''
  JHEP {\bf 0005}, 021 (2000)
  [arXiv:hep-ph/0005080];
  %%CITATION = JHEPA,0005,021;%%
%\cite{Grossman:2003gq}
%\bibitem{Grossman:2003gq}
  Y.~Grossman and S.~Rakshit,
  %``Neutrino masses in R-parity violating supersymmetric models,''
  Phys.\ Rev.\  D {\bf 69}, 093002 (2004)
  [arXiv:hep-ph/0311310].
  %%CITATION = PHRVA,D69,093002;%%


%\cite{Diaz:2006ee}
\bibitem{Diaz:2006ee}
  M.~A.~Diaz, P.~Fileviez Perez and C.~Mora,
  %``Neutrino Masses in Split Supersymmetry,''
  Phys.\ Rev.\  D {\bf 79}, 013005 (2009)
  [arXiv:hep-ph/0605285].
  %%CITATION = PHRVA,D79,013005;%%

%\cite{Diaz:2009yz}
\bibitem{Diaz:2009yz}
  M.~A.~Diaz, B.~Koch, B.~Panes,
  %``Gravity Effects on Neutrino Masses in Split Supersymmetry,''
  Phys.\ Rev.\  {\bf D79}, 113009 (2009).
  [arXiv:0902.1720 [hep-ph]].

\bibitem{Sundrum:2009gv}
  R.~Sundrum,
  %``SUSY Splits, But Then Returns,''
  JHEP {\bf 1101}, 062 (2011)
  [arXiv:0909.5430 [hep-th]].
  %%CITATION = JHEPA,1101,062;%%


\bibitem{Diaz:2009gf}
  M.~A.~Diaz, F.~Garay and B.~Koch,
  %``Explaining Solar Neutrinos with Heavy Higgs Masses in Partial Split
  %Supersymmetry,''
  Phys.\ Rev.\  D {\bf 80}, 113005 (2009)
  [arXiv:0910.2987 [hep-ph]].
  %%CITATION = PHRVA,D80,113005;%%

%\cite{Diaz:2011pc}
\bibitem{Diaz:2011pc}
  M.~A.~Diaz, S.~G.~Saenz and B.~Koch,
  %``Gravitino Dark Matter and Neutrino Masses in Partial Split Supersymmetry,''
  Phys.\ Rev.\  D {\bf 84}, 055007 (2011)
  [arXiv:1106.0308 [hep-ph]].
  %%CITATION = PHRVA,D84,055007;%%

\bibitem{Choi:2010jt}
  K.~Y.~Choi, D.~Restrepo, C.~E.~Yaguna and O.~Zapata,
  %``Indirect detection of gravitino dark matter including its three-body
  %decays,''
  JCAP {\bf 1010}, 033 (2010)
  [arXiv:1007.1728 [hep-ph]].
  %%CITATION = JCAPA,1010,033;%%

\bibitem{Choi:2010xn}
  K.~Y.~Choi and C.~E.~Yaguna,
  %``New decay modes of gravitino dark matter,''
  Phys.\ Rev.\  D {\bf 82}, 015008 (2010)
  [arXiv:1003.3401 [hep-ph]].
  %%CITATION = PHRVA,D82,015008;%%

\bibitem{arXiv:1106.0308}
  M.~A.~Diaz, S.~G.~Saenz and B.~Koch,
  %``Gravitino Dark Matter and Neutrino Masses in Partial Split Supersymmetry,''
  Phys.\ Rev.\  D {\bf 84}, 055007 (2011)
  [arXiv:1106.0308 [hep-ph]].
  %%CITATION = PHRVA,D84,055007;%%

\bibitem{Buchmuller:2007ui}
  W.~Buchmuller, L.~Covi, K.~Hamaguchi, A.~Ibarra and T.~Yanagida,
  %``Gravitino Dark Matter in R-Parity Breaking Vacua,''
  JHEP {\bf 0703}, 037 (2007)
  [arXiv:hep-ph/0702184].
  %%CITATION = JHEPA,0703,037;%%

\bibitem{Navarro:1995iw}
  J.~F.~Navarro, C.~S.~Frenk and S.~D.~M.~White,
  %``The Structure of cold dark matter halos,''
  Astrophys.\ J.\  {\bf 462}, 563 (1996)
  [arXiv:astro-ph/9508025].
  %%CITATION = ASJOA,462,563;%%

%\cite{Bertone:2007aw}
\bibitem{Bertone:2007aw}
  G.~Bertone, W.~Buchmuller, L.~Covi and A.~Ibarra,
  %``Gamma-Rays from Decaying Dark Matter,''
  JCAP {\bf 0711}, 003 (2007)
  [arXiv:0709.2299 [astro-ph]].
  %%CITATION = JCAPA,0711,003;%%

\bibitem{Abdo:2010nz}
  A.~A.~Abdo {\it et al.}  [The Fermi-LAT collaboration],
  %``The Spectrum of the Isotropic Diffuse Gamma-Ray Emission Derived From
  %First-Year Fermi Large Area Telescope Data,''
  Phys.\ Rev.\ Lett.\  {\bf 104}, 101101 (2010)
  [arXiv:1002.3603 [astro-ph.HE]].
  %%CITATION = PRLTA,104,101101;%%


%\cite{Restrepo:2011rj}
\bibitem{Restrepo:2011rj}
  D.~Restrepo, M.~Taoso, J.~W.~F.~Valle and O.~Zapata,
  %``Gravitino dark matter and neutrino masses with bilinear R-parity
  %violation,''
  arXiv:1109.0512 [hep-ph].
  %%CITATION = ARXIV:1109.0512;%%
  
  %\cite{Huang:2011xr}
\bibitem{Huang:2011xr}
  X.~Huang, G.~Vertongen and C.~Weniger,
  %``Probing Dark Matter Decay and Annihilation with Fermi LAT Observations of
  %Nearby Galaxy Clusters,''
  arXiv:1110.1529 [hep-ph].
  %%CITATION = ARXIV:1110.1529;%%
 
%\cite{GomezVargas:2011ph}
\bibitem{GomezVargas:2011ph}
  G.~A.~Gomez-Vargas, M.~Fornasa, F.~Zandanel, A.~J.~Cuesta, C.~Munoz, F.~Prada and G.~Yepes,
  %``CLUES on Fermi-LAT prospects for the extragalactic detection of munuSSM
  %gravitino Dark Matter,''
  arXiv:1110.3305 [astro-ph.HE].
  %%CITATION = ARXIV:1110.3305;%%

\bibitem{Weinberg:1979sa}
  S.~Weinberg,
  %``Baryon and Lepton Nonconserving Processes,''
  Phys.\ Rev.\ Lett.\  {\bf 43}, 1566 (1979).
  %%CITATION = PRLTA,43,1566;%%


\bibitem{hep-ph/9701253}
  M.~Hirsch, H.~V.~Klapdor-Kleingrothaus and S.~G.~Kovalenko,
  %``B-L violating masses in softly broken supersymmetry,''
  Phys.\ Lett.\  B {\bf 398}, 311 (1997)
  [arXiv:hep-ph/9701253].
  %%CITATION = PHLTA,B398,311;%%


\end{thebibliography}



==> Author/BenjaminKochpre.tex <==
%Benjamin Koch$^{*a}$, Marco Aurelio D\'\i az$^{a}$, and Sebasti\'an Garc\'ia S\'aenz$^{a}$,

%$^{*}$ speaker

%$^a$ Pontificia Universidad Catolica Chile

%\begin{center}
{\bf Abstract}\\
%\vskip5.mm
We discuss the decays of
gravitinos in the model of partial split supersymmetry (PSS),
finding that for a large range of gravitino masses, the
two body decay channel is dominant.
Taking the gravitino as dark matter candidate 
and demanding that the model also describes the established
neutrino masses and mixings we show that one can derive
a theoretical upper limit for the gravitino mass within
this model. Finally we address questions that have been
raised during this workshop.
%\end{center}

\vskip5.mm

\section{introduction}
Split supersymmetry (SS) was originally proposed to address two of the most 
conspicuous 
problems of supersymmetric models, which are fast proton decay and excessive 
flavor changing neutral currents and CP violation \cite{ArkaniHamed:2004fb}. In
SS the 
solution to these problems is 
accomplished by considering all squarks and sleptons very massive, with a mass
scale 
$\widetilde m$ somewhere between the supersymmetric scale $M_{susy}$ and the
Grand 
Unification scale $M_{GUT}$. One of the Higgs bosons remains light, as usual in 
supersymmetric models, as well as the gauginos and higgsinos, with all these
particles 
having a mass accessible to the LHC \cite{Aad:2009wy}.
In addition to this,
the introduction of bilinear R-parity violation into this kind of
models allows for a rich phenomenology, especially in the neutrino sector
\cite{Barbier:2004ez,Nowakowski:1995dx,Hirsch:2000ef,Chun:2004mu,Diaz:2006ee,Diaz:2009yz,Sundrum:2009gv}.

A variation of this model is 
Partial Split Supersymmetry (PSS). In PSS all squarks and sleptons have a mass
of the order of
the SS mass scale $\widetilde m$, but both Higgs doublets remain with a mass at
the electroweak scale \cite{Diaz:2006ee,Sundrum:2009gv}. The addition of RpV to
this
model was introduced to be able to generate a solar neutrino 
mass \cite{Diaz:2006ee}. Loop contributions from neutral CP-even and CP-odd 
Higgs bosons are indeed able to do the job, producing not only the atmospheric
and solar masses, but also the atmospheric, solar, and reactor neutrino mixing 
angles \cite{Diaz:2009gf}.

In R-parity violating PSS the usual dark matter candidates
of supersymmetric models (the neutralinos) are unstable. 
However, the gravitino is an alternative to the neutralino.
Also the gravitino can decay into standard model particles,
but its decay is expected to be further suppressed by the
Planck mass $M_P$. This proceedings paper is essentially
a summary of \cite{Diaz:2011pc}.

\section{Partial Split Supersymmetry}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In PSS both Higgs doublets remain with a mass at the electroweak scale. As
it happens in SS, higgsinos, gauginos, and Higgs bosons interact via induced 
R-parity conserving couplings of the type,
%
\begin{eqnarray}
{\cal L}_{PSS}^{RpC} &\owns& 
-\textstyle{\frac{1}{\sqrt{2}}} H_u^\dagger
(\tilde g_u \sigma\widetilde W + \tilde g'_u\widetilde B)\widetilde H_u
-\textstyle{\frac{1}{\sqrt{2}}} H_d^\dagger
(\tilde g_d \sigma \widetilde W - \tilde g'_d \widetilde B)\widetilde H_d 
+\mathrm{h.c.},
\label{RpCterms}
\end{eqnarray}
%
where $\tilde g_u$, $\tilde g'_u$, $\tilde g_d$, and $\tilde g'_d$ are
couplings induced in the effective low energy lagrangian. At the SS scale
$\widetilde m$ they satisfy the boundary conditions,
%
$\tilde g_u=\tilde g_d=g\,,\qquad \tilde g'_u=\tilde g'_d=g'$,
evolving with independent RGE down to the electroweak scale. Similarly to the
MSSM, both Higgs fields acquire a vacuum expectation value $\langle H_u\rangle=v_u$
and $\langle H_d\rangle=v_d$, with the constraint 
$v^2=v_u^2+v_d^2=246\,{\mathrm{GeV}}^2$
and the definition $\tan\beta=v_u/v_d$. Gauginos and higgsinos mix forming the
neutralinos, with a mass matrix very similar to the one in the MSSM.
The relevant bi-linear R-parity violating couplings are
\begin{equation}
{\cal L}_{PSS}^{RpV} =
-\epsilon_i \widetilde H_u^T \epsilon L_i  
\ -\ 
\textstyle{\frac{1}{\sqrt{2}}} b_i H_u^T\epsilon
(\tilde g_d \sigma\widetilde W-\tilde g'_d\widetilde B)L_i 
\ + \ h.c., 
\label{LSS2HDMRpV}
\end{equation}
where the $b_i$ are the parameters of the lepton-higgs-gaugino interactions,
$\epsilon=i\sigma_2$, and the $\epsilon_i$ are the supersymmetric BRpV
parameters.
The effective neutrino mass matrix in this approach was found to be \cite{Diaz:2009gf}
%
\begin{equation}
{\bf M}_\nu|_{ij}=A\Lambda_i\Lambda_j+
C\epsilon_i\epsilon_j,
\quad  \mbox{with}\quad 
\Lambda_i=\mu b_i v_u+\epsilon_i v_d\quad,
\label{DpiH2HDM}
\end{equation}
%
where
%
\begin{equation}
A^{(0)}= \frac{M_1 \tilde g^2_d + M_2 \tilde g'^2_d}{4\det{M_{\chi^0}}}.
\label{A0}
\end{equation}
and where the coefficient $C$ arises from loop diagrams with virtual
mixed Higgs fields and neutralinos.
The theoretical background model will be further discussed in  a later section.
In order to make a connection with neutrino physics we will now turn
to the photino-neutrino mixing in this model $U_{\tilde \gamma \nu}$.
This mixing is governed by the same parameters as neutrino mass matrix.
Thus, imposing that the model fits neutrino data reduces the 
parameter space of PSS which translates into an allowed range for the
mixing $U_{\tilde \gamma \nu}$. The determination of this range
was done numerically. For example for $M_1=300\,$GeV one finds
\begin{equation}
2 \cdot 10^{-17}<U_{\tilde \gamma \nu}<3 \cdot 10^{-14}\quad.
\end{equation}
This range will be of importance in the context of gravitino decay.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Gravitino Decay and Induced Photon flux}

In R-parity violating models the gravitino can decay completely
into ordinary particles which should lead to an observable
signature from gravitino dark matter. In our calculations
of this signature we asume that$m_{3/2}<m_W$.

The first coupling that is relevant for gravitino decay is
\begin{equation} \label{coupleGravi}
{\cal L} \owns -\frac{1}{4M_P} \overline\psi_\mu \sigma^{\nu\rho}
\gamma^\mu \lambda_\gamma F_{\nu\rho}
\end{equation}
%
where $M_P$ is the Planck mass, $\psi_\mu$ is the spin-$3/2$ gravitino 
field, $\lambda_\gamma$ is the spin-$1/2$ photino field, 
$F_{\nu\rho}=\partial_\nu A_\rho-\partial_\rho A_\nu$ is the photon field
strength, and $A_\mu$ is the photon field.
This coupling gives rise to a vertex gravitino photon, photino.
Due to a violation of R-parity the photino can further transform into a 
neutrino. This tranforation is proportional to the mixingo between
photino and neutrino $U_{\tilde \gamma \nu}$.
The resulting two body decay rate is then
\begin{equation} \label{eq:2body}
\Gamma(\widetilde{G}\rightarrow\gamma\nu) = 
\frac{m_{3/2}^3}{32\pi M_P^2}|{U}_{\widetilde{\gamma}\nu}|^2.
\end{equation}
In PSS the mixing between photon and photino is
\begin{equation} \label{eq:gammamixing}
U_{\widetilde{\gamma}\nu_i}\simeq\frac{\mu}{2({\rm det}M_{\chi^0})} 
\left(\tilde{g}_dM_1s_W-\tilde{g}'_dM_2c_W\right)\Lambda_i.
\end{equation}
The constants here are parameters of PSS which are also relevant
for the generation of neutrino masses and mixings within this model.

In addition to this two body decay one has to take into account
also the possible three body decays.
When studying the three body decay a more general part
of the interaction Lagrangian comes into play
\bea\label{coupleGravi2}
{\mathcal{L}}&\owns&
-\frac{i}{\sqrt{2}M_P}\left[
(D^*_\mu\phi^{i*})\bar \psi_\nu \gamma^\mu \gamma^\nu P_L \chi^i-
(D_\mu \phi^i)\bar \chi^i P_R \gamma^\nu \gamma^\mu \psi_\nu
\right]\\ \nonumber
&&-\frac{i}{8 M_P}\bar \psi_\mu 
\left[ \gamma^\nu,\gamma^\rho\right]
\gamma^\mu \lambda^{(\alpha)a}F_{\nu \rho}^{(\alpha)a}\quad,
\eea
where the second line is in analogy to (\ref{coupleGravi}) and the first line
introduces additional couplings with scalar fields $\phi$.
The 3-body decays of the gravitino were studied in detail for the first time in 
\cite{Choi:2010jt,Choi:2010xn}, where explicit formulae are given. Nevertheless,
our calculations 
have yielded that the three-body results in \cite{Choi:2010jt} have to be
corrected.
We agree, however, with the conclusion that the 3-body decays are indeed
important, 
and cannot be neglected in general.
The interaction (\ref{coupleGravi2}) allows for various amplitdes that
contribute to the decay of a gravitino into a neutrino and two leptons with
opposite charge. The details of this calculation were given in
\cite{arXiv:1106.0308}. 
We find 3-body decay branching ratios for small gravitino
masses $m_{3/2}<20\,$GeV of the
order of $<15\%$.

If dark matter consists of those gravitinos, their
decays should contribute to the photon spectra observed 
by astrophysical experiments.
This contribution consists of a 
mono-energetic line of energy $m_{3/2}/2$ from the two-body decay, plus a 
continuum distribution from the three-body decays. The exact form of the 
spectrum, which depends on $m_{3/2}$ and $M_1$, was studied in detail in 
\cite{Choi:2010jt,Choi:2010xn} using an event generator. 
Since the first contribution is the dominant feature \cite{Buchmuller:2007ui}
only this will be considered.
Here we are interested
in obtaining constraints on the gravitino parameters, for which it suffices 
as an approximation to consider only the photon line from the two-body 
decay, as this is the most prominent feature of the spectrum for values 
of $M_1$ up to 1 TeV \cite{Choi:2010jt}.
Following established models of dark matter distribution
and photon flux propagation
\cite{Navarro:1995iw,Bertone:2007aw,Buchmuller:2007ui}
one obtains the diffenctial flux in dependence of the photon energy
due to (\ref{eq:2body}). This flux, which is supposed
to be strongly peaked at the gravitino mass, can be compared
to the photon flux from the same region of the sky, which was
measured by the Fermi LAT collaboration \cite{Abdo:2010nz}.
Since the observed flux does not show any strong peak,
this non-observation can be used to constrain the parameters 
of the decay rate (\ref{eq:2body}). This method is essentially analogous
to   \cite{Restrepo:2011rj,Huang:2011xr,GomezVargas:2011ph}.
One obtains
\begin{equation} \label{eq:constraint1}
\left(\frac{\tau_{3/2}}{10^{27}~{\rm s}}\right)>\frac{0.851}{p(m_{3/2})}
B(\widetilde{G}\rightarrow\gamma\nu) 
\left(\frac{m_{3/2}}{1~{\rm GeV}}\right)^{\gamma-2},
\end{equation}
where we parametrized the energy dependent resolution for the Fermi LAT
experiment
$\sigma=m_{3/2}p(m_{3/2})/2$ by
\begin{equation}
p(m_{3/2}) = 0.349-0.142\log\left(\frac{m_{3/2}}{2~
{\rm MeV}}\right)+0.019\log^2\left(\frac{m_{3/2}}{2~{\rm MeV}}\right).
\end{equation}
In equation (\ref{eq:constraint1}) further appears
the two body branching ratio of the gravitino decay $B$ and
the lifetime of the  gravitino $\tau_{3/2}$.

Now we are in place to combine the constraints from the neutrino
sector and from the observed photon spectrum.
Both constraints can be visualized in a $m_{3/2}-\tau_{3/2}$ plane as it is 
shown in figure \ref{fig1ben}.
\begin{center}
\begin{figure}[h!]
\includegraphics[width=8cm]{Author/r300p.pdf}
\caption{\it Allowed region for $M_1=300$ GeV}
\label{fig1ben}
\end{figure}
\end{center}
From this figure one can also read off the essential conclusion
of this study: PSS as a model for neutrino mass and the possibility
of gravitino dark matter leads to the prediction of an upper limit
of the gravitino mass in the range of $10\,$GeV.

\section{Questions and answers }
We would like use the remaining space to address some questions 
that were raised during the workshop. We appreciate those comments
because they lead to a better understanding of the basic mechanism
at work.
\begin{itemize}
\item {\it``A dimension five operator generating $\nu$-Majorana masses
needs to have (i) lepton number violation and (ii) it needs
to be proportional to the square of a $SU(2)_L$ breaking vacuum expectation value \cite{Weinberg:1979sa}. Are both conditions fulfilled?''}

Both conditions are fulfilled. Condition (i) is rather obvious due to the Majorana nature
of the term in the effective Lagrangian. The vacuum expectation value of condition (ii)
is somewhat hidden in the $C$-term of the equation \ref{DpiH2HDM} which
can be shown to be proportional to $m_Z^2$.
\item  {\it``In m-sugra a vanishing splitting between the real and imaginary s-neutrino
masses drives two of the three neutrino masses to zero. The same should
happen in this model where the s-neutrinos are integrated out''}

The splitting is controlled by the value of $\epsilon(i)B(i)\rightarrow B_{\epsilon}^i$
which in general does not necessarily have to be as small as in m-sugra.
Actually in PSS it is not small.
The reason for this to happen can be seen in equation (B7)
of the paper \cite{Diaz:2006ee}:
If one assumes very large s-neutrino masses $M_{Li}$
this tadpole equation demands equally large values of
$B_{\epsilon}^i \sim v_i M_{Li}^2/v_u$. Thus the mixing parameter
grows in such a way that the Higgses and the s-neutrinos
always mix. As it can be seen in equations (44,45) of the same
paper: The matching conditions between PSS and MSSM at the
large scale $\tilde{m}$ imply that this mixing has a definite value
$s_s^i\sim c_{\alpha}v_i/v_u$ .
There are also no problems from the side of the mass bounds
since the charged scalar/sbottom loops are suppressed by
the large mass scale of the sbottom. 

\item {\it There is a theorem in \cite{hep-ph/9701253} that states:
  If the real part and the imaginary part of the s-neutrino
have equal values $m_{sn Re}=m_{sn Im}$ then the
Majorana like B-L violating mass term has to vanish
which again implies neutrinos have to have zero mass $m_nu=0$. 
Is there a contradiction?}

No there is no contradiction.
The $m_H$ and the $m_A$ Higgses have a fixed
part of s-neutrino (as explained above), thus the general
statement of that paper predicts for the case of PSS: 
If $m_H=m_A$, then $m_\nu =0$;
That this statement is true can be seen from
\cite{Diaz:2009gf}:
Equations (12,13) of this paper show that
$m_H^2\approx m_A^2 +m_Z^2 sin^2(2 \beta)$,
thus the splitting is $\sim m_Z^2 sin^2(2 \beta)$.
However as one can see from equation (23) of the
same paper: If this splitting is zero, then also the
contribution to $m_\nu$ is zero.
This is the realization of the general statement in PSS. 

\item 
{\it It has been shown that: If there is no s-neutrino 
then there is no neutrino Majorana mass \cite{hep-ph/9701253}.
Is there a contradiction?}

No there is no contradiction.
Since the s-neutrinos mix with the Higgses due to
the possibly large parameter $B_\epsilon^i$ there is always
a part of the s-neutrino interaction eigenstates in PSS.
Thus, there is no contradiction with this theorem.
\end{itemize}

\begin{thebibliography}{9}
\bibitem{ArkaniHamed:2004fb}
  N.~Arkani-Hamed and S.~Dimopoulos,
  %``Supersymmetric unification without low energy supersymmetry and signatures
  %for fine-tuning at the LHC,''
  JHEP {\bf 0506}, 073 (2005)
  [arXiv:hep-th/0405159];
  %%CITATION = JHEPA,0506,073;%%
%\cite{Giudice:2004tc}
%\bibitem{Giudice:2004tc}
  G.~F.~Giudice and A.~Romanino,
  %``Split supersymmetry,''
  Nucl.\ Phys.\  B {\bf 699}, 65 (2004)
  [Erratum-ibid.\  B {\bf 706}, 65 (2005)]
  [arXiv:hep-ph/0406088].

\bibitem{Aad:2009wy}
  G.~Aad {\it et al.}  [The ATLAS Collaboration],
  %``Expected Performance of the ATLAS Experiment - Detector, Trigger and
  %Physics,''
  arXiv:0901.0512 [hep-ex].
  %%CITATION = ARXIV:0901.0512;%%

%\cite{Barbier:2004ez}
\bibitem{Barbier:2004ez}
  R.~Barbier {\it et al.},
  %``R-parity violating supersymmetry,''
  Phys.\ Rept.\  {\bf 420}, 1 (2005)
  [arXiv:hep-ph/0406039].
  %%CITATION = PRPLC,420,1;%%

%\cite{Nowakowski:1995dx}
\bibitem{Nowakowski:1995dx}
  M.~Nowakowski and A.~Pilaftsis,
  %``W and Z boson interactions in supersymmetric models with explicit R-parity
  %violation,''
  Nucl.\ Phys.\  B {\bf 461}, 19 (1996)
  [arXiv:hep-ph/9508271];
  %%CITATION = NUPHA,B461,19;%%
%\cite{Hempfling:1995wj}
%\bibitem{Hempfling:1995wj}
  R.~Hempfling,
  %``Neutrino Masses and Mixing Angles in SUSY-GUT Theories with explicit
  %R-Parity Breaking,''
  Nucl.\ Phys.\  B {\bf 478}, 3 (1996)
  [arXiv:hep-ph/9511288].
  %%CITATION = NUPHA,B478,3;%%

%\cite{Hirsch:2000ef}
\bibitem{Hirsch:2000ef}
  M.~Hirsch, M.~A.~Diaz, W.~Porod, J.~C.~Romao and J.~W.~F.~Valle,
  %``Neutrino masses and mixings from supersymmetry with bilinear R-parity
  %violation: A theory for solar and atmospheric neutrino oscillations,''
  Phys.\ Rev.\  D {\bf 62}, 113008 (2000)
  [Erratum-ibid.\  D {\bf 65}, 119901 (2002)]
  [arXiv:hep-ph/0004115].
  %%CITATION = PHRVA,D62,113008;%%

%\cite{Chun:2004mu}
\bibitem{Chun:2004mu}
  E.~J.~Chun and S.~C.~Park,
  %``Neutrino mass from R-parity violation in split supersymmetry,''
  JHEP {\bf 0501}, 009 (2005)
  [arXiv:hep-ph/0410242];
  %%CITATION = JHEPA,0501,009;%%
%\cite{Davidson:2000ne}
%\bibitem{Davidson:2000ne}
  S.~Davidson and M.~Losada,
  %``Basis independent neutrino masses in the R(p) violating MSSM,''
  Phys.\ Rev.\  D {\bf 65}, 075025 (2002)
  [arXiv:hep-ph/0010325];
  %%CITATION = PHRVA,D65,075025;%%
%\cite{Davidson:2000uc}
%\bibitem{Davidson:2000uc}
  S.~Davidson and M.~Losada,
  %``Neutrino masses in the R(p) violating MSSM,''
  JHEP {\bf 0005}, 021 (2000)
  [arXiv:hep-ph/0005080];
  %%CITATION = JHEPA,0005,021;%%
%\cite{Grossman:2003gq}
%\bibitem{Grossman:2003gq}
  Y.~Grossman and S.~Rakshit,
  %``Neutrino masses in R-parity violating supersymmetric models,''
  Phys.\ Rev.\  D {\bf 69}, 093002 (2004)
  [arXiv:hep-ph/0311310].
  %%CITATION = PHRVA,D69,093002;%%


%\cite{Diaz:2006ee}
\bibitem{Diaz:2006ee}
  M.~A.~Diaz, P.~Fileviez Perez and C.~Mora,
  %``Neutrino Masses in Split Supersymmetry,''
  Phys.\ Rev.\  D {\bf 79}, 013005 (2009)
  [arXiv:hep-ph/0605285].
  %%CITATION = PHRVA,D79,013005;%%

%\cite{Diaz:2009yz}
\bibitem{Diaz:2009yz}
  M.~A.~Diaz, B.~Koch, B.~Panes,
  %``Gravity Effects on Neutrino Masses in Split Supersymmetry,''
  Phys.\ Rev.\  {\bf D79}, 113009 (2009).
  [arXiv:0902.1720 [hep-ph]].

\bibitem{Sundrum:2009gv}
  R.~Sundrum,
  %``SUSY Splits, But Then Returns,''
  JHEP {\bf 1101}, 062 (2011)
  [arXiv:0909.5430 [hep-th]].
  %%CITATION = JHEPA,1101,062;%%


\bibitem{Diaz:2009gf}
  M.~A.~Diaz, F.~Garay and B.~Koch,
  %``Explaining Solar Neutrinos with Heavy Higgs Masses in Partial Split
  %Supersymmetry,''
  Phys.\ Rev.\  D {\bf 80}, 113005 (2009)
  [arXiv:0910.2987 [hep-ph]].
  %%CITATION = PHRVA,D80,113005;%%

%\cite{Diaz:2011pc}
\bibitem{Diaz:2011pc}
  M.~A.~Diaz, S.~G.~Saenz and B.~Koch,
  %``Gravitino Dark Matter and Neutrino Masses in Partial Split Supersymmetry,''
  Phys.\ Rev.\  D {\bf 84}, 055007 (2011)
  [arXiv:1106.0308 [hep-ph]].
  %%CITATION = PHRVA,D84,055007;%%

\bibitem{Choi:2010jt}
  K.~Y.~Choi, D.~Restrepo, C.~E.~Yaguna and O.~Zapata,
  %``Indirect detection of gravitino dark matter including its three-body
  %decays,''
  JCAP {\bf 1010}, 033 (2010)
  [arXiv:1007.1728 [hep-ph]].
  %%CITATION = JCAPA,1010,033;%%

\bibitem{Choi:2010xn}
  K.~Y.~Choi and C.~E.~Yaguna,
  %``New decay modes of gravitino dark matter,''
  Phys.\ Rev.\  D {\bf 82}, 015008 (2010)
  [arXiv:1003.3401 [hep-ph]].
  %%CITATION = PHRVA,D82,015008;%%

\bibitem{arXiv:1106.0308}
  M.~A.~Diaz, S.~G.~Saenz and B.~Koch,
  %``Gravitino Dark Matter and Neutrino Masses in Partial Split Supersymmetry,''
  Phys.\ Rev.\  D {\bf 84}, 055007 (2011)
  [arXiv:1106.0308 [hep-ph]].
  %%CITATION = PHRVA,D84,055007;%%

\bibitem{Buchmuller:2007ui}
  W.~Buchmuller, L.~Covi, K.~Hamaguchi, A.~Ibarra and T.~Yanagida,
  %``Gravitino Dark Matter in R-Parity Breaking Vacua,''
  JHEP {\bf 0703}, 037 (2007)
  [arXiv:hep-ph/0702184].
  %%CITATION = JHEPA,0703,037;%%

\bibitem{Navarro:1995iw}
  J.~F.~Navarro, C.~S.~Frenk and S.~D.~M.~White,
  %``The Structure of cold dark matter halos,''
  Astrophys.\ J.\  {\bf 462}, 563 (1996)
  [arXiv:astro-ph/9508025].
  %%CITATION = ASJOA,462,563;%%

%\cite{Bertone:2007aw}
\bibitem{Bertone:2007aw}
  G.~Bertone, W.~Buchmuller, L.~Covi and A.~Ibarra,
  %``Gamma-Rays from Decaying Dark Matter,''
  JCAP {\bf 0711}, 003 (2007)
  [arXiv:0709.2299 [astro-ph]].
  %%CITATION = JCAPA,0711,003;%%

\bibitem{Abdo:2010nz}
  A.~A.~Abdo {\it et al.}  [The Fermi-LAT collaboration],
  %``The Spectrum of the Isotropic Diffuse Gamma-Ray Emission Derived From
  %First-Year Fermi Large Area Telescope Data,''
  Phys.\ Rev.\ Lett.\  {\bf 104}, 101101 (2010)
  [arXiv:1002.3603 [astro-ph.HE]].
  %%CITATION = PRLTA,104,101101;%%


%\cite{Restrepo:2011rj}
\bibitem{Restrepo:2011rj}
  D.~Restrepo, M.~Taoso, J.~W.~F.~Valle and O.~Zapata,
  %``Gravitino dark matter and neutrino masses with bilinear R-parity
  %violation,''
  arXiv:1109.0512 [hep-ph].
  %%CITATION = ARXIV:1109.0512;%%
  
  %\cite{Huang:2011xr}
\bibitem{Huang:2011xr}
  X.~Huang, G.~Vertongen and C.~Weniger,
  %``Probing Dark Matter Decay and Annihilation with Fermi LAT Observations of
  %Nearby Galaxy Clusters,''
  arXiv:1110.1529 [hep-ph].
  %%CITATION = ARXIV:1110.1529;%%
 
%\cite{GomezVargas:2011ph}
\bibitem{GomezVargas:2011ph}
  G.~A.~Gomez-Vargas, M.~Fornasa, F.~Zandanel, A.~J.~Cuesta, C.~Munoz, F.~Prada and G.~Yepes,
  %``CLUES on Fermi-LAT prospects for the extragalactic detection of munuSSM
  %gravitino Dark Matter,''
  arXiv:1110.3305 [astro-ph.HE].
  %%CITATION = ARXIV:1110.3305;%%

\bibitem{Weinberg:1979sa}
  S.~Weinberg,
  %``Baryon and Lepton Nonconserving Processes,''
  Phys.\ Rev.\ Lett.\  {\bf 43}, 1566 (1979).
  %%CITATION = PRLTA,43,1566;%%


\bibitem{hep-ph/9701253}
  M.~Hirsch, H.~V.~Klapdor-Kleingrothaus and S.~G.~Kovalenko,
  %``B-L violating masses in softly broken supersymmetry,''
  Phys.\ Lett.\  B {\bf 398}, 311 (1997)
  [arXiv:hep-ph/9701253].
  %%CITATION = PHLTA,B398,311;%%


\end{thebibliography}



==> Author/Hagedorn-old.tex <==
%Author: C. Hagedorn
%Title: Continuous and Discrete (Flavor)  Symmetries
%Affilliation: Istituto Nazionale di Fisica Nucleare, Sezione di Padova, via Marzolo, 8, 35131 Padua, Italy
%Acknowledgements: I would like to warmly thank the organizers of this workshop for giving me the opportunity to present this talk
%as well as for the nice and stimulating atmosphere during the workshop.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{center}
{\bf Abstract}\\
\vskip5.mm
In this talk I give an overview over continuous and discrete groups and how these are used in the field of model 
building as flavor symmetries. The latter act on the space of the three generations of elementary particles. I mainly 
concentrate on discussing generic mathematical properties of these groups relevant for understanding their possible 
predictive power when applied to explain fermion mass and mixing patterns. I also put emphasis on the 
classification of discrete groups.
%\end{center}

\vskip5.mm

\section{Introduction}
The existence of three generations of elementary  particles is well-established. They can be  distinguished according to their mass as well as their mixing. 
The mass hierarchy among charged fermions is known to be strong, especially in the up quark sector
\begin{equation}\nonumber
m_u: m_c: m_t \approx \lambda^8: \lambda^4: 1 \;\; , \;
m_d: m_s: m_b\approx \lambda^4: \lambda^2: 1 \;\; , \;
m_e: m_\mu: m_\tau\approx \lambda^{4\div 5}: \lambda^2: 1 \;\;\; \mbox{with} \;\;\; \lambda \approx 0.22 \, ,
\end{equation}
while it is much milder in the neutrino sector. Neutrino masses are experimentally constrained by the measurements of solar and 
atmospheric mass square differences (at the $2 \sigma$ level) \cite{fogli}
\begin{equation}\nonumber
\delta m^2 \equiv \Delta m^2_{\mathrm{sol}} \equiv m_2^2 - m_1^2 = (7.58 ^{+0.41} _{-0.42}) \, \times \, 10^{-5} \, \mathrm{eV}^2
\;\; , \;
|\Delta m^2| \equiv \left| m_3^2 - \frac{m_2^2+m_1^2}{2} \right|= (2.35 ^{+0.22} _{-0.18}) \, \times \, 10^{-3} \, \mathrm{eV}^2 \, .
\end{equation} 
The sign of $\Delta m^2$ is undetermined and the absolute neutrino mass scale $m_0$ is bounded, $m_0 \lesssim 0.3 \, \mathrm{eV}$, by cosmological measurements \cite{cosmo}, searches for
neutrinoless double beta \cite{0nubb} and Tritium beta decay \cite{Tritium}. 
The mixing among quarks is small 
\begin{equation}\nonumber
\theta_{12} ^{q} \equiv \theta_{C} \approx 13 ^{\circ} \; , \;\;
\theta_{23} ^{q} \approx 2.4 ^{\circ} \;\;\; \mbox{and} \;\;\; \theta _{13} ^{q} \approx 0.21 ^{\circ} \, .
\end{equation}
At the same time, lepton mixing, measured in neutrino oscillation experiments, involves
two large mixing angles \cite{fogli}
\begin{equation}\nonumber
\sin^2 \theta_{12}^l=0.306^{+0.036}_{-0.031}  \; , \;\; \sin^2 \theta_{23}^l=0.42^{+0.18}_{-0.06} \;\;\; (2 \sigma \, \mbox{level})
\end{equation}
and a third small angle which is non-zero \cite{fogli}  - according to recent experimental indications \cite{T2K} 
\begin{equation}
\sin^2 \theta_{13}^l =0.021^{+0.015}_{-0.013}  \;\;\; (2  \sigma \, \mbox{level}) \, .
\end{equation}
This value is obtained using the old estimates for reactor anti-neutrino fluxes.
Neither the hierarchy among the charged fermion masses nor the fermion mixing patterns can be explained in the framework 
of the Standard Model (SM).  The peculiar structure of the lepton mixing is compatible
with special, theoretically motivated, patterns like
\begin{itemize}
\item $\mu\tau$ symmetric mixing \cite{mutau}: $\sin ^{2} \theta _{23}^{l} = \frac{1}{2} \; , \;\;\; \sin ^{2} \theta _{13}^{l} = 0\;\;$ and $\;\; \theta_{12}^l \sim {\cal O}(1)$,
\item tri-bimaximal (TB) mixing \cite{HPS}:  $\sin^{2} \theta _{12}^{l} = \frac{1}{3} \; , \;\;\; \sin ^{2} \theta _{23}^{l} = \frac{1}{2} \; ,
\;\;\; \sin ^{2} \theta _{13}^{l} = 0$,
\item golden ratio pattern \cite{GR}: $\sin^{2} \theta _{12}^{l} = \frac{1}{\sqrt{5} \phi} \approx 0.276 \; , \;\; \sin ^{2} \theta _{23}^{l} = \frac{1}{2} \; , \;\;\; \sin ^{2} \theta _{13}^{l} = 0$
with $\phi=( 1+ \sqrt{5})/2$,
\item bimaximal mixing \cite{BMorg}:   $\sin^{2} \theta _{12}^{l} = \frac{1}{2} \; , \;\;\; \sin ^{2} \theta _{23}^{l} = \frac{1}{2} \; , \;\;\; \sin ^{2} \theta _{13}^{l} = 0$,
\end{itemize}
up to small corrections. Taking into consideration the success of symmetries describing correctly the gauge interactions of the SM particles,
it is tempting to assume a flavor symmetry $G_f$, i.e. a symmetry acting on the space of generations, to be responsible for the features of fermion masses and mixing.

In section \ref{sec2} I present an overview over general properties of a flavor symmetry $G_f$. Section \ref{sec3} is dedicated to a brief discussion of models with continuous $G_f$
and section \ref{sec4} contains the explanation of the connection between the non-trivial symmetry breaking of a discrete group $G_f$ and the fermion mixing pattern.
I show how TB mixing
arises from the groups $A_4$ and $S_4$ and how predictions for elements of the mixing matrix are derived from (single-valued and double-valued) dihedral groups. In section \ref{sec5} I 
sketch a supersymmetric $D_{14}$ model explaining the Cabibbo angle $\theta_C$ and its extension to the lepton sector which leads to maximal atmospheric mixing,
vanishing $\theta_{13}^l$ and generically large $\theta_{12}^l$. I conclude in section \ref{sec6}.

\mathversion{bold}
\section{General properties of $G_f$}
\label{sec2}
\mathversion{normal}

Several properties of this new symmetry have to be fixed, namely 
\begin{itemize}
\item whether it is abelian or non-abelian,
\item whether it is continuous (like the gauge symmetries) or discrete (like parity), 
\item whether it is local (like the gauge symmetries) or global (like lepton number $U(1)_L$),
\item whether it commutes with the other symmetries (e.g. gauge symmetries) of the theory or not,
\item whether it is broken spontaneously or explicitly,
\item whether it is broken at high energies (like at the seesaw or the GUT scale) or low energies (like the electroweak scale),
\item whether it is broken in an arbitrary way or to one of its subgroups. 
\end{itemize}
Apart from that the size of $G_f$ depends on the gauge group of the model, e.g. in the framework of the SM without right-handed neutrinos
the maximal symmetry of the kinetic terms of the fermions is $U(3)^5$, while it is reduced to $U(3)$ in the case of an $SO(10)$ model in which
all fermions of one generation including the right-handed neutrino are unified into the 16-dimensional representation.

The presence of more than one generation can only be explained with a non-abelian symmetry which has two- and three-dimensional irreducible
representations. An advantage of discrete over continuous symmetries is that the former in general contain several small representations suitable to host
the three fermion generations. Furthermore, it is well-known that the spontaneous breaking of a continuous global (local) symmetry leads to the appearance of Goldstone (gauge) bosons, 
respectively. In order to avoid this I choose the symmetry to be discrete. However, also the breaking of the latter does in general lead to experimentally constrained effects,
namely the generation of domain walls. This does not pose a problem as long as the scale at which the symmetry is broken is comparable with or larger than
the scale of inflation. Thus high energy scales like the seesaw scale or the scale of grand unification seem to be preferred. In this case the flavor symmetry $G_f$ is usually
broken through non-vanishing vacuum expectation values (VEVs) of gauge singlets, called flavons. Models in which $G_f$ is broken at a low energy scale contain instead
several Higgs doublets which also transform non-trivially under $G_f$. Such models seem to be disfavored, because flavor changing neutral
currents and lepton flavor violating processes, like $\mu\to e\gamma$, are induced. Another possibility is to explicitly break $G_f$, for example, at the boundaries of an extra spatial dimension.

A list of possible choices for $G_f$ is
\begin{itemize}
\item continuous symmetries: $SU(2)$, $U(2)$, $SO(3)$, $SU(3)$ and $U(3)$.
\item discrete symmetries:
\begin{itemize}
\item permutation symmetries: symmetric groups $S_N$ and alternating groups $A_N$ 
with $N \in \mathbb{N}$,
\item dihedral symmetries: single-valued groups $D_n$ and double-valued groups $D'_n$ 
with $n \in \mathbb{N}$,
\item further double-valued groups: $T'$, $O'$, $I'$, ...
\item subgroups of $SU(3)$: $\Delta (3 \, n^2)$ and $\Delta (6 \, n^2)$ with $n \in \mathbb{N}$, as well
as $\Sigma$ groups,
\item subgroups of $U(3)$ such as $\Sigma(81)$ or of the listed groups, e.g. $T_7 \cong Z_7 \rtimes Z_3 \subset \Delta (147)$.
\end{itemize}
\end{itemize}

\mathversion{bold}
\section{Overwiev over models with continuous $G_f$}
\label{sec3}
\mathversion{normal}

In this section I give a brief, and incomplete, survey over models with continuous non-abelian flavor symmetries.
In \cite{U2} supersymmetric models with a $U(2)$ group are discussed in the context of $SU(5)$ and $SO(10)$ grand unified theories (GUTs). Generic features of these models are: 
 the three generations of fermions are assigned to ${\bf 2} + {\bf 1}$ which easily explains the heaviness of the third generation and allows
 to alleviate the so-called supersymmetric flavor problem; the breaking of the symmetry $U(2)$ proceeds in
 two steps, first to a $U(1)$ subgroup and then to nothing. These models predict nine relations among fermion masses and mixing, however,
 only $\theta_{23}^l$ is in general large in the lepton sector, while the two other mixing angles $\theta_{12}^l$ and $\theta_{13}^l$ are small.
 Models with flavor symmetries $SO(3)$ \cite{SO3} and $SU(3)$ \cite{SU3} are more promising, because they allow to unify all three generations of elementary
 particles. Furthermore, the largeness of two mixing angles, $\theta_{12}^l$ and $\theta_{23}^l$, in the lepton sector indicates that all
 three generations are closely related instead of only two. Also in these models the breaking of the flavor symmetry proceeds usually in two
 steps, i.e. $SO(3) \to SO(2) \to \mbox{nothing}$ and $SU(3) \to SU(2) \to \mbox{nothing}$, respectively. The models are supersymmetric and 
the  gauge group is the one of the SM, the Pati-Salam group or, in the case of an extra-dimensional model, $SO(10)$. The masses of the SM fermions arise
usually only from non-renormalizable operators and additional symmetries, such as $Z_n$ or $U(1)$, are imposed in order to forbid certain operators.
Assuming different messenger mass scales allows to differentiate among the expansion parameters present in the up quark, down quark and charged lepton
mass matrices. It has been shown that in such models TB neutrino mixing is predicted through constrained sequential dominance and
a specific structure of the flavons VEVs. The latter can be achieved through F- as well as D-terms. The corrections arising
from the charged lepton sector to the mixing angles are small. Subsequently, models in which the continuous symmetry has been replaced by
a discrete one, like $A_4$, $\Delta(27)$ and $\Delta(108)$, have been discussed \cite{SU3disc}. The results of these models are very similar to those with continuous
flavor groups. In general, the vacuum alignment is achieved in a simpler way; however, in the case of a discrete group D-terms associated with 
the flavor symmetry are obviously absent.

\mathversion{bold}
\section{Non-trivial breaking of discrete $G_f$ and fermion mixing}
\label{sec4}
\mathversion{normal}

In the following I exemplify the idea of the non-trivial breaking of the flavor symmetry in different sectors of the theory, e.g. the charged lepton and the neutrino
one, presenting several models: first, I briefly discuss how $A_4$ and $S_4$ give rise to TB mixing, then dihedral symmetries $D_n$ in general
as well as the group $D_{14}$ in particular which can explain quark and lepton mixing patterns at the same time.

\mathversion{bold}
\subsection{TB mixing and the groups $A_4$ and $S_4$}
\mathversion{normal}

Probably, one of the most famous examples of a flavor symmetry broken in a non-trivial way is the one of the group $A_4$ which leads to the prediction of 
TB mixing. A simple and elegant model can be found in \cite{AF2}. It is an extension of the minimal supersymmetric SM (MSSM) in which the group $A_4$ is spontaneously
broken at high energies through flavon VEVs. The theory is formulated as an effective one with a cutoff $\Lambda$, assumed to be of the order 
of the GUT scale. An elaborate construction of the potential ensures
the correct vacuum alignment. The supermultiplets containing left-handed leptons transform as irreducible triplet of $A_4$ and right-handed charged leptons are
in three inequivalent one-dimensional representations. The two Higgs doublets $h_{u,d}$ do not transform under $A_4$, while the flavons breaking $A_4$ correctly
are two triplets, called $\varphi_T$ and $\varphi_S$ and two singlets $\xi$, $\tilde \xi$ (only one of them acquires a non-zero VEV). Apart from $A_4$
the model has a family independent $Z_3$ symmetry and a family dependent $U(1)_{FN}$ symmetry.
The former allows to separate the two sets of flavons $\{ \varphi_T \}$ and $\{ \varphi_S, \xi, \tilde\xi \}$ and thus
the charged lepton and neutrino sectors in the superpotential at the renormalizable level, while the latter which distinguishes among the right-handed charged leptons
is used to explain the hierarchy among charged lepton masses. This $U(1)_{FN}$ symmetry is also assumed to be spontaneously broken, by a gauge singlet $\theta$, carrying
charge $-1$. 

The group $A_4$ is the symmetry group of the even permutations of four objects and is isomorphic to the symmetry group of a regular tetrahedron. It has 12 elements and
four irreducible representations: three singlets $1$, $1'$, $1''$ and a triplet $3$. The only non-trivial Kronecker product is $3 \times 3 = 1+1'+1''+ 3+3$. The group
can be defined in terms of two generators $S$ and $T$ which satisfy the relations ($E$ is the neutral element of the group) \cite{AF2}
\begin{equation}
\label{A4rel}
S^{2}=E \; , \;\;\; T^{3}=E \; , \;\;\; (ST)^{3} =E \, .
\end{equation}
For the singlets $S$ and $T$ are simply $1$ and the third roots of unity, $1$, $\omega^2$, $\omega$, respectively. For the triplet we use a basis in which $T$ is represented
through a diagonal matrix \cite{AF2}
\begin{equation}
S=\frac{1}{3}\left(\begin{array}{ccc}
       -1 & 2 & 2 \\
       2  & -1 & 2\\
       2  & 2 & -1 \\
       \end{array}\right) \;\;\; , \;\;\; T=\left(\begin{array}{ccc}
                                   1 & 0 & 0 \\
                                   0 & \omega^2 & 0 \\
                                   0 & 0 & \omega \\
                               \end{array}\right) \, .
\end{equation}
With the vacuum alignment (for details see \cite{AF2})
\begin{equation}
\langle \varphi_S \rangle = v_S \left(1,1,1 \right) \;\; , \;\; \langle \xi \rangle = u \;\; , \;\; \langle \tilde\xi\rangle =0  \;\; , \;\; \langle\varphi_T\rangle = v_T \left( 1,0,0 \right) \;\; ,
\end{equation}
the mass matrix ${\cal M}_l$ of the charged leptons is diagonal
\begin{equation}
{\cal M}_l =\frac{v_{T}}{\Lambda} \langle h_d \rangle \; \mbox{diag} 
			\left( y_e \, \frac{\langle \theta \rangle ^2}{\Lambda^2}, 
                         y_\mu \, \frac{\langle \theta \rangle}{\Lambda}, y_\tau \right) \, ,
\end{equation}
while the one of the neutrinos $M_\nu$ arising from the Weinberg operator takes the form
\begin{equation}
\label{MnuA4}
M_\nu=\frac{\langle h_u \rangle^2}{\Lambda}\left(
\begin{array}{ccc}
a+2 b/3& -b/3& -b/3\\
-b/3& 2b/3& a-b/3\\
-b/3& a-b/3& 2 b/3
\end{array}
\right) \, .
\end{equation}
As one immediately sees the latter leads to TB mixing and the neutrino masses are $|a+b|$, $|a|$, $|-a+b|$ in units of $\langle h_u \rangle^2/\Lambda$ with 
$a=x_{a} \, u/\Lambda$, $b=x_{b} \, v_{S}/\Lambda$.
Apart from its simplicity this model is very appealing, because, as has been observed, the group $A_4$ is broken in a specific way. The flavons $\varphi_S$ ($\xi$) break
$A_4$ to a $Z_2$ subgroup in the neutrino sector, since the VEVs of these flavons are eigenvectors to the eigenvalue +1 of the element $S$ of $A_4$. 
From eq.(\ref{A4rel}) it is obvious that $S$ generates
a $Z_2$ group. The VEV of $\varphi_T$ breaks $A_4$ to a $Z_3$ subgroup in the charged lepton sector, because it is an eigenvector to the eigenvalue +1 of the matrix representing the element $T$
of $A_4$ which has order three, see eq.(\ref{A4rel}). Note that in this way $A_4$ is broken completely in the whole theory. The mismatch of the two different subgroups of $A_4$, preserved in 
neutrino and charged lepton sectors, reflects the mismatch between neutrinos and charged leptons  in the flavor space and thus allows for a neat interpretation of lepton mixing.
All this is independent of the particular value of the fermion masses. Similarly, small mixing in the quark sector might be understood as sign that the subgroups preserved in
the up and down quark sectors are the same (for a model realizing this idea with the help of the group $T'$, the double covering of $A_4$, see \cite{FHLM07}).

From the mathematical point of view two things are interesting to notice:
first of all, not only non-zero VEVs of fields forming a $1$ or a $3$ can preserve a $Z_2$ group, but also those of fields transforming as $1'$ or $1''$, and second, apart from 
$Z_2$ and $Z_3$  $D_2$ is a subgroup of $A_4$ (whose preservation is however only compatible with non-zero VEVs of flavons being singlets of $A_4$).
The first aspect can be seen in a different way: the matrix in eq.(\ref{MnuA4}) is not only invariant under the element $S$ of $A_4$, but also under the matrix $P_{23}$ which
is the matrix representing the permutation of second and third rows and columns. The latter generates also a $Z_2$ group and commutes with the element $S$. Thus,
the neutrino mass matrix $M_\nu$ is invariant under $Z_2 \times Z_2$, with one of the two being a subgroup of $A_4$, while the other one is an accidental symmetry which
arises through the particular choice of the flavor symmetry breaking fields. This fact has been used as argument against $A_4$ and 
it has been shown \cite{Lam0708} that indeed from the mathematical view point the group $S_4$ is more appropriate for predicting TB mixing, because it contains the element
$S$ as well as $P_{23}$. The simple idea is then to use $S_4$ as flavor group and break it to $Z_2 \times Z_2$ in the neutrino sector, while the breaking in the charged lepton
sector remains the same, i.e. $S_4 \to Z_3$. Again, the flavor group is broken completely in the whole theory. However, one problem which might arise in $S_4$ models is 
related to the question of how to achieve the mass hierarchy among charged leptons naturally, because $S_4$ only contains two inequivalent singlets in contrast to $A_4$. Thus,
it might not be simple to distinguish the three (right-handed) charged leptons. This problem can however be easily solved \cite{CHMS1} by
extending the flavor group to $S_4 \times Z_3$ and breaking the latter in the charged lepton sector to $Z_3^{(D)}$ which is the diagonal subgroup of the external $Z_3$ factor
and the $Z_3$ contained in $S_4$ and generated by $T$. In order to distinguish the three right-handed charged leptons which transform trivially
under $S_4$, one assigns them to $1$, $\omega^2$ and $\omega$ under the additional $Z_3$ group.

Before discussing other flavor groups let me briefly comment on the question whether or not models predicting TB mixing
are still favored in the light of the recent experimental results \cite{T2K} which indicate a non-zero value for $\theta_{13}^l$. Indeed, in all models the leading order result, in this case
TB mixing, receives corrections from various sources, e.g. higher-dimensional operators. Thus, in all models a non-zero value of $\theta_{13}^l$ is aspected. Concerning its size one can
roughly say: let us assume the size of the corrections to be $\delta$ and that the latter contribute in the same manner to all three mixing angles, then the request to not perturb
too much the result for the solar mixing angle implies that $\delta \lesssim 0.05$. Thus, one might expect $\sin\theta_{13}^l \sim \delta \lesssim 0.05$ which is too small to explain the
recent experimental indication. Since in many models several operators give rise to a correction to $\theta_{13}^l$,  we get in general $\sin\theta_{13}^l \approx |c| \delta$ with $c$ complex.
If $c$ is largish, i.e. the corrections add up, larger values of $\theta_{13}^l$ can be explained. Alternatively, one can consider models in which the corrections to the reactor mixing 
angle are generically larger than to the two other angles. This happens for example if there are two sets of flavor symmetry breaking fields whose VEVs are different in size 
\cite{Lin09}. Yet, another possibility is to assume that the mixing pattern at leading order is bimaximal mixing. Then, the reactor as well as the solar mixing angle have to receive corrections of 
order $\delta \sim \lambda \sim 0.2$ \cite{S4BM}. The crucial issue is then to protect the atmospheric mixing angle $\theta_{23}^l$ from too large corrections.


\mathversion{bold}
\subsection{Dihedral symmetries $D_n$ as $G_f$}
\mathversion{normal}

In order to show the interesting and amusing properties, a non-trivial breaking of a discrete symmetry can have, I discuss the case of a dihedral flavor group $D_n$
which is broken to two distinct $Z_2$ subgroups. If the former is generated by $\rm A$ and $\rm B$, the generating elements of the latter are $\mathrm{B A}^{k_1}$
and $\mathrm{B A}^{k_2}$ ($k_i$ integers), respectively. If two of the left-handed fermion (quark or lepton) generations transform as irreducible two-dimensional representation ${\bf \underline{2}}_{\rm j}$,
one of the elements of the mixing matrix $V$ is of the form
\begin{equation}
|V_{\alpha\beta}|= \left| \cos \left( \frac{\pi \, (k_{1} - k_{2}) \, \mathrm{j}}{n} \right) \right| \, .
\label{Vab}
\end{equation}
As one can nicely see, $|V_{\alpha\beta}|$ only depends on group-theoretical quantities, i.e. the index $n$ of the dihedral group $D_n$, the indices characterizing the two $Z_2$
subgroups $k_{1,2}$ and the index $\rm j$ of the two-dimensional representation. Note that for $k_1=k_2$ the mixing is trivial, as 
expected. The way to reach the result in eq.(\ref{Vab}) can be understood performing the following seven steps: first, one has to choose the group $D_n$ and select the indices $k_{1,2}$ of the two
$Z_2$ subgroups which are associated with the two different fermion sectors 1 and 2. Then, one assigns left-handed fields to ${\bf \underline{1}}_{\rm s} + {\bf \underline{2}}_{\rm j}$, while
the three generations of right-handed fermions can either transform as singlets ${\bf \underline{1}_{\rm i_p}}$ or also as singlet and doublet ${\bf \underline{1}}_{\rm l} + {\bf \underline{2}}_{\rm m}$.
We then consider a generic model in which two sets of scalars exist $\{\Phi_1\}$ and $\{\Phi_2\}$. These sets contain fields in all representations $\mu$ of $D_n$ and we assume their VEVs to be
such that they leave invariant a $Z_2$ group generated by $\mathrm{B A}^{k_{1,2}}$, respectively. As one can check, the most general matrices ${\cal M}_i$ with $i=1,2$ for fermions of sector
1 and 2 are of the form (always given in the left-right basis)
\begin{equation}
\label{Mp1}
\mathcal{M}_i = \left( \begin{array}{ccc}
  0 & A_i & B_i \\
  C_i & D_i & E_i\\
  -C_i \mathrm{e}^{- i \varphi_i \mathrm{j}} & D_i \mathrm{e}^{- i \varphi_i \mathrm{j}}
& E_i \mathrm{e}^{- i \varphi_i \mathrm{j}}
\end{array}
\right) \, ,
\end{equation}
if right-handed fermions are singlets under the group $D_n$, or take the form
\begin{equation} 
\label{Mp2}
\mathcal{M}_i = \left( \begin{array}{ccc}
  A_i & C_i & C_i \mathrm{e}^{- i \varphi_i \mathrm{m}}\\
  B_i & D_i & E_i\\
  B_i \mathrm{e}^{- i \varphi_i \mathrm{j}} & E_i \mathrm{e}^{- i \varphi_i (\mathrm{j}-\mathrm{m})}
& D_i \mathrm{e}^{- i \varphi_i (\mathrm{j}+\mathrm{m})}
\end{array}
\right) \, ,
\end{equation}
if right-handed fermions transform as ${\bf \underline{1}}_{\rm l} + {\bf \underline{2}}_{\rm m}$. The parameters $A_i$,...,$E_i$ are in general complex and not further constrained
by the flavor symmetry $D_n$. The phase $\varphi_i$ which appears in both cases only depends on group-theoretical
quantities
\begin{equation}
\varphi_i = \frac{2 \pi k_i}{n} \, .
\end{equation} 
For both matrices the combination ${\cal M}_i {\cal M}_i^\dagger$ can be written as
\begin{equation}
\label{MMd}
\mathcal{M}_i \mathcal{M}_i^\dagger= \left( \begin{array}{ccc}
  a_i & b_i \mathrm{e}^{i \zeta_i} & b_i \mathrm{e}^{i (\zeta_i + \varphi_i \mathrm{j})}\\
  b_i \mathrm{e}^{- i \zeta_i} & c_i & d_i \mathrm{e}^{i \varphi_i \mathrm{j}}\\
  b_i \mathrm{e}^{- i (\zeta_i+\varphi_i \mathrm{j})} & d_i \mathrm{e}^{- i \varphi_i \mathrm{j}} & c_i 
\end{array}
\right) 
\end{equation}
with $a_i$,...,$d_i$ and $\zeta_i$ depending on the parameters present in the matrices in eqs.(\ref{Mp1})-(\ref{Mp2}).
The matrix $U_i$ diagonalizing the combination ${\cal M}_i {\cal M}_i^\dagger$ is
\begin{equation}
U_i = \left( \begin{array}{ccc}
 0 & \cos \theta_i \, \mathrm{e} ^{i \zeta_i}& \sin \theta_i \, \mathrm{e}^{i \zeta_i}\\   
 - \frac{1}{\sqrt{2}} \mathrm{e}^{i \varphi_i \mathrm{j}} & - \frac{\sin \theta_i}{\sqrt{2}} & \frac{\cos\theta_i}{\sqrt{2}}\\
 \frac{1}{\sqrt{2}}  & - \frac{\sin \theta_i}{\sqrt{2}} \mathrm{e}^{-i \varphi_i \mathrm{j}} & \frac{\cos\theta_i}{\sqrt{2}}
\mathrm{e}^{-i \varphi_i \mathrm{j}}
\end{array}
\right) 
\end{equation}
with $\theta_{i}$ given in terms of the parameters appearing in eq.(\ref{MMd}).
As one clearly sees, one of the eigenvectors only contains the phase $\varphi_i$ and thus only depends on group-theoretical quantities. The physical mixing arises from the misalignment of the
matrices $U_1$ and $U_2$:
\begin{equation}
V=U_1^\dagger U_2 \; .
\end{equation}
Then one of the elements $|V_{\alpha\beta}|$ is of the form
\begin{equation}
|V_{\alpha\beta}| = \frac{1}{2} \left| 1 + \mathrm{e}^{i (\varphi_1 -\varphi_2) \mathrm{j}}\right|
= \left|\cos \left( (\varphi_1 -\varphi_2) \frac{\mathrm{j}}{2} \right) \right|
= \left| \cos \left( \frac{\pi \, (k_{1} - k_{2}) \, \mathrm{j}}{n} \right) \right| \, ,
\end{equation}
while the rest depends also on the angles $\theta_{1,2}$ and the phases $\zeta_{1,2}$.

It has been shown \cite{BHL07}  that $\mu\tau$ symmetric lepton mixing can be realized in this way with the group $D_4$ \cite{myD4}
and that $D_{14}$ can be used to predict the correct size of the Cabibbio angle \cite{BH09}. In the subsequent section a model is outlined
in which $D_{14}$ plays the role of the flavor symmetry and which explains the Cabibbo angle as well as nearly $\mu\tau$
symmetric lepton mixing \cite{HMD14}.

\mathversion{bold}
\section{$D_{14}$ - a symmetry for quarks and leptons}
\label{sec5}
\mathversion{normal}

The group $D_{14}$ belongs to the dihedral symmetries and has 28 elements. As all $D_n$ groups, it only contains one- and two-dimensional representations, called
${\bf \underline{1}}_{{\rm i}}$, ${\rm i}=1,...,4$ and ${\bf \underline{2}}_{{\rm j}}$, ${\rm j}=1,...,6$. It can be described in  terms of two generators $\rm A$ and $\rm B$ which satisfy the relations
\begin{equation}
{\rm A}^{14} = E \; , \;\; {\rm B}^{2} = E \; , \;\; \rm A \, B \, A = B \, .
\end{equation}
The generators $\rm A$ and $\rm B$ for the singlets are just $\pm 1$ and the two-by-two matrices for ${\bf \underline{2}}_{{\rm j}}$ are in a convenient basis
\begin{equation}
\rm A =\left(\begin{array}{cc} 
                           \mathrm{e}^{\left( \frac{\pi i}{7} \right) \, \mathrm{j}} & 0 \\
                            0 & \mathrm{e}^{-\left( \frac{\pi i}{7} \right)
                              \, \mathrm{j}} 
          \end{array}\right) \;\;\;\; \mbox{and} \;\;\;\; \rm B=\left(\begin{array}{cc} 
                                       0 & 1 \\
                                       1 & 0 
                  \end{array}\right) \; .
\end{equation}

The main properties of the original $D_{14}$ model \cite{BH09} which only contains quarks are the following: 
it is an extension of the MSSM formulated as effective theory with a cutoff $\Lambda$, the flavor symmetry $G_f$ is the product $D_{14} \times U(1)_{FN} \times Z_3$, $D_{14}$ and $U(1)_{FN}$ together explain
the quark mass hierarchies and $Z_3$ is used for separating appropriately up and down quark sectors. All flavor symmetries are broken spontaneously at high energies through flavon VEVs. 
The two sets of flavons breaking the group $D_{14} \times Z_3$ are $\{ \psi^{u}_{1,2}, \chi_{1,2}^{u}, \xi^{u}_{1,2}, \eta^{u} \}$ and 
$\{ \psi^{d}_{1,2}, \chi_{1,2}^{d}, \xi^{d}_{1,2}, \eta^{d}, \sigma \}$, while $\theta$ only carries non-trivial $U(1)_{FN}$ charge. The left-handed quark doublets 
$Q_{D}=(Q_1, Q_2)$ and $Q_3$ are in the representations ${\bf \underline{2}}_1$ and ${\bf \underline{1}}_1$, while the right-handed quarks $u^c$, $c^c$, $t^c$ and $d^c$, $s^c$, $b^c$ are singlets under $D_{14}$
and $h_{u,d}$ are trivial singlets of $D_{14}$.

The leading operators contributing to up quark masses are (order one coefficients are omitted in the following and $(\cdots)$ denotes the contraction to a $D_{14}$-invariant)
\begin{eqnarray}
&&Q_3 \, t^c \, h_u +  \frac{1}{\Lambda} (Q_D \psi^u)  t^c h_u + \frac{1}{\Lambda} Q_3 (c^c \eta^u) h_u\\
&+& \frac{\theta^2}{\Lambda^4} (Q_D u^c \chi^u \xi^u) h_u + \frac{\theta^2}{\Lambda^4} \left(Q_D u^c (\xi^u)^2 \right) h_u + \frac{\theta^2}{\Lambda^4} (Q_D  \psi^u \eta^u u^c) h_u\\
&+& \frac{1}{\Lambda^2} (Q_D c^c \chi^u \xi^u)  h_u + \frac{1}{\Lambda^2} \left(Q_D c^c (\xi^u)^2 \right) h_u + \frac{1}{\Lambda^2} (Q_D  \psi^u) (\eta^u c^c) h_u \, ,
\end{eqnarray}
while the ones contributing to the masses of the down quarks read
\begin{equation}
\frac{1}{\Lambda} Q_3 (b^c \eta^d) h_d + \frac{\theta}{\Lambda^2} \, Q_3 \, s^c \sigma h_d + \frac{\theta}{\Lambda^2} \, (Q_D \psi^d) \, s^c h_d \, .
\end{equation}
Note that all these operators respect the separation among the up and down quark sectors, as up-type flavons only contribute to up quark masses and down-type ones only to down quark masses. 
With the appropriate vacuum configuration of the flavons, see \cite{BH09} for details of the superpotential, two distinct $Z_2$ groups
are preserved. One is characterized with an even index, see above,  which can be set without loss of generality to zero, while the second one has an odd index $k$ which remains undetermined.
At the $Z_2$ symmetry preserving level, the up and down quark mass matrices are of the form
\begin{equation}
\mathcal{M}_u = \left(
\begin{array}{ccc}
	- \alpha^u_1 \, t^2 \, \epsilon^2  & \alpha^u_2 \, \epsilon^2 
				& \alpha^u_3 \, \epsilon \\
	\alpha^u_1 \, t^2 \, \epsilon^2 & \alpha^u_2 \, \epsilon^2 & \alpha^u_3 \, \epsilon\\
	0 & \alpha^u_4 \, \epsilon & y_t 
\end{array}
\right) \, \langle h_u \rangle \;\;\; \mbox{and} \;\;\;
\mathcal{M}_d = \left(
\begin{array}{ccc}
	 0 & \alpha^d_1 \, t \, \epsilon  & 0\\
	 0 & \alpha^d_1 \, \mathrm{e} ^{- \pi i k/7} \, t \, \epsilon & 0 \\
	 0 & \alpha^d_2 \, t \, \epsilon & y_b \, \epsilon 
\end{array}
\right) \, \langle h_d \rangle 
\end{equation}
with $\langle\Phi^u\rangle/\Lambda \approx \epsilon$, $\langle\Phi^d\rangle/\Lambda \approx \epsilon$, $t = \langle\theta\rangle/\Lambda \approx \epsilon \approx \lambda^2 \approx 0.04$.
As one easily computes, the quark masses fulfill the relations
\begin{eqnarray}
m_u^2:m_c^2:m_t^2 &\sim& \epsilon^8: \epsilon^4: 1 \; , \;\; m_d^2:m_s^2:m_b^2  \sim 0: \epsilon^2: 1 \; ,\\ \nonumber
m_b^2:m_t^2 &\sim& \epsilon^2:1 \;\;\; \mbox{for} \;\;\; \mbox{small} \;\;\; \tan\beta = \langle h_u \rangle/\langle h_d \rangle
\end{eqnarray}
and the CKM mixing matrix takes the form
\begin{equation}
|V_{CKM}|  = \left( 
\begin{array}{ccc}
	|\cos (\frac{k \, \pi}{14})| & |\sin (\frac{k \, \pi}{14})| & 0 \\
	|\sin (\frac{k \, \pi}{14})| & |\cos (\frac{k \, \pi}{14})| & 0\\
	0   		             & 0			    & 1
\end{array}
\right) +
\left( 
\begin{array}{ccc}
	0  			& \mathcal{O}(\epsilon^4) 	& \mathcal{O}(\epsilon^2)  \\
	\mathcal{O}(\epsilon^2)	& \mathcal{O}(\epsilon^2)	& \mathcal{O}(\epsilon)    \\
	\mathcal{O}(\epsilon) 	& \mathcal{O}(\epsilon)		& \mathcal{O}(\epsilon^2)
\end{array}
\right)  \, .
\end{equation}
As one can see, for the choices $k=1$ and $k=13$ the matrix elements involving the first two generations are very close to their experimental best fit values, e.g.  $|V_{ud}| \approx 0.97493$
should be compared with $|V_{ud}|_{\rm exp} = 0.97419 ^{+0.00022} _{-0.00022}$. Subleading corrections lead to the down quark mass of the correct size as well as allow all
elements of $V_{CKM}$ and the Jarlskog invariant $J_{CP}$ to be accommodated.

In a second step I would like to outline how to extend this model to the lepton sector in a minimalistic way, i.e. to add only a small number of new fields, to not perturb
the results achieved for quarks too much and at the same time to predict $\mu\tau$ symmetric lepton mixing. The setup which fulfills these requirements is the following \cite{HMD14}: the $Z_3$ factor 
of the flavor symmetry is replaced by $Z_7$ and still has the role to segregate the different symmetry breaking sectors, the left-handed leptons $L_1$ and $L_D=(L_2, L_3)$ transform 
as ${\bf \underline{1}}_3$ and ${\bf \underline{2}}_2$, also
the right-handed neutrinos $\nu^c_1$ and $\nu^c_D=(\nu^c_2, \nu^c_3)$ transform 
as ${\bf \underline{1}}_2 + {\bf  \underline{2}}_3$, while all right-handed charged leptons $e^c$, $\mu^c$, $\tau^c$ are trivial singlets of
$D_{14}$. Furthermore, one flavon $\chi^e_{1,2}$ is added which is a doublet ${\bf \underline{2}}_2$ of $D_{14}$.

In the neutrino sector, the leading contributions to the right-handed neutrino mass matrix ${\cal M}_R$ are
\begin{equation}
 \nu^c_1 \nu^c_1 \sigma + (\nu^c_D \nu^c_D) \sigma
\;\;\;\;\;\; \mbox{giving rise to} \;\;\;\;\;\; 
\mathcal{M}_R = \left( \begin{array}{ccc}
 \alpha^M_1 & 0 & 0\\
 0 & 0 & \alpha^M_2\\
 0 & \alpha^M_2 & 0
\end{array}
\right) \, \epsilon \, \Lambda \; ,
\end{equation}
while the Dirac neutrino mass matrix ${\cal M}^D_\nu$ takes the form
\begin{equation}
\mathcal{M}^D_\nu = \left( \begin{array}{ccc}
 0 & \alpha^D_1 & \alpha^D_1\\
\alpha^D_ 2 & 0 & \alpha^D_3\\
-\alpha^D_2 & \alpha^D_3 & 0
\end{array}
\right) \, \epsilon \, \langle h_u \rangle
\end{equation}
and receives at leading level contributions from the operators
\begin{equation}
\frac{1}{\Lambda}  (L_1 \nu_D^c \xi^u) h_u +  \frac{1}{\Lambda} (L_D \nu_1^c \chi^u)  h_u +  \frac{1}{\Lambda} (L_D \nu_D^c \psi^u) h_u \, .
\end{equation}
Consequently, the light neutrino mass matrix $\mathcal{M}_\nu$ can be cast into the form
\begin{equation}
\mathcal{M}_\nu = \left( \begin{array}{ccc}
  2 x^2/v & x & x \\
 x & z & v-z\\
 x & v-z & z
\end{array}
\right) \, \epsilon \, \langle h_u \rangle^2/\Lambda \, .
\end{equation}
The predictions are then: $\mu\tau$ symmetric neutrino mixing, $\tan (\theta_{12}^\nu) = \sqrt{2}\left|\frac{x }{v} \right|$ and
normal ordering with $m_1=0$. 
In addition, one finds $|m_{ee}| = m_2 \, \sin^2 (\theta_{12}^\nu) = \sqrt{\delta m^2} \, \sin^2 (\theta_{12}^\nu)$.
For the charged lepton sector we use the additional flavon $\chi^e_{1,2}$ which acquires a VEV of the form $v^e \, (1,0)$. Such an alignment is easily achieved
with a driving field being a trivial singlet under $D_{14}$ and carrying an appropriate $Z_7$ charge. Interestingly enough, also this alignment preserves a
$Z_2$ subgroup of $D_{14}$ which, however, does not coincide with one of the $Z_2$ symmetries present in the up and down quark sectors. The main contributions
to the charged lepton mass matrix ${\cal M}_l$ originate from ($\alpha$ stands for $e$, $\mu$ and $\tau$)
\begin{equation}
 \frac{1}{\Lambda} (L_D \chi^e) \, \alpha^c \, h_d + \frac{1}{\Lambda^2} (L_D \chi^e \xi^u) \, \alpha^c \, h_d
 + \frac{1}{\Lambda^3} (L_1 \chi^e \psi^u \xi^u) \alpha^c h_d+ \frac{1}{\Lambda^3} (L_1 \eta^u) (\chi^e \chi^u) \alpha^c h_d
\end{equation}
which give rise to
\begin{equation}
\mathcal{M}_l = \left( \begin{array}{ccc}
		\alpha^e_1 \, \epsilon^3 & \alpha^e_2 \, \epsilon^3 & \alpha^e_3 \, \epsilon^3\\
		\alpha^e_4 \, \epsilon^2 & \alpha^e_5 \, \epsilon^2 & \alpha^e_6 \, \epsilon^2\\
		\alpha^e_7 \, \epsilon & \alpha^e_8 \, \epsilon & \alpha^e_9 \, \epsilon
\end{array}
\right) \langle h_d \rangle \;\;\;\;\;\;\;\;\; \mbox{for} \;\;\;\;\; v^e/\Lambda \approx \epsilon \approx \lambda^2 \, .
\end{equation}
As one can see, the charged lepton mass hierarchy is correctly predicted,  $m_e : m_\mu : m_\tau \sim \epsilon^2 : \epsilon : 1$,
and the three mixing angles in the charged lepton sector are small
\begin{equation}
\theta_{12}^e \sim \epsilon \, , \,\, \theta_{13}^e \sim \epsilon^2 \, , \,\, \theta_{23}^e \sim \epsilon \, .
\end{equation}
Thus, the lepton mixing is nearly $\mu\tau$ symmetric, i.e.
\begin{equation}
\sin^2 \theta_{23}^l = \frac{1}{2} + \mathcal{O}(\epsilon) \; , \;\; \sin \theta_{13}^l = \mathcal{O}(\epsilon) \, , \;\; \sin^2 \theta_{12}^l = \mathcal{O}(1) \, .
\end{equation}
As regards the recent indication for $\theta_{13}^l \neq 0$ \cite{T2K}, we note that the model naturally leads only to rather small $\theta_{13}^l$ which might seem to be disfavored
at the moment.

\section{Conclusions}
\label{sec6}

I have presented an overview over flavor symmetries in general and their properties. I commented briefly on the case of a continuous $G_f$ and then focussed on discrete symmetries
playing the role of $G_f$ with special emphasis on those cases in which they are broken in a non-trivial way. I showed a variety of examples: $A_4$ and $S_4$ and their relation to TB mixing,
predictions from dihedral groups $D_n$ in general and from $D_{14}$ in particular. Lastly, I have sketched a $D_{14}$ model in which the Cabibbo angle as well as $\mu\tau$ symmetric lepton
mixing are closely related to how $D_{14}$ is broken and at the same time all fermion mass hierarchies are naturally accommodated.

\begin{thebibliography}{9}

\bibitem{fogli}
  G.~L.~Fogli, E.~Lisi, A.~Marrone, A.~Palazzo and A.~M.~Rotunno,
  %``Evidence of $\theta_{13}$>0 from global neutrino data analysis,''
  Phys.\ Rev.\ D\ {\bf 84} (2011) 053007
  [arXiv:1106.6028 [hep-ph]].
  %%CITATION = PHRVA,D84,053007;%%

\bibitem{cosmo}
G.~L.~Fogli, E.~Lisi, A.~Marrone, A.~Melchiorri, A.~Palazzo, A.~M.~Rotunno, P.~Serra and J.~Silk {\it et al.},
  %``Observables sensitive to absolute neutrino masses. 2.,''
  Phys.\ Rev.\ D\ {\bf 78} (2008) 033010
  [arXiv:0805.2517 [hep-ph]].
  %%CITATION = PHRVA,D78,033010;%%

\bibitem{0nubb}
J.~J.~Gomez-Cadenas, J.~Martin-Albo, M.~Mezzetto, F.~Monrabal and M.~Sorel,
  %``The Search for neutrinoless double beta decay,''
  %Submitted to: Riv.Nuovo Cim.
  arXiv:1109.5515 [hep-ex].
  %%CITATION = RNCIB,,;%%

\bibitem{Tritium}
C.~Kraus, B.~Bornschein, L.~Bornschein, J.~Bonn, B.~Flatt, A.~Kovalik, B.~Ostrick and E.~W.~Otten {\it et al.},
  %``Final results from phase II of the Mainz neutrino mass search in tritium beta decay,''
  Eur.\ Phys.\ J.\ C\ {\bf 40} (2005) 447
  [hep-ex/0412056];
  %%CITATION = EPHJA,C40,447;%%
V.~M.~Lobashev,
  %``The search for the neutrino mass by direct method in the tritium beta-decay and perspectives of study it in the project KATRIN,''
  Nucl.\ Phys.\ A\ {\bf 719} (2003) 153.
  %%CITATION = NUPHA,A719,153;%%

\bibitem{T2K}
  K.~Abe {\it et al.} [T2K Collaboration],
  %``Indication of Electron Neutrino Appearance from an Accelerator-produced Off-axis Muon Neutrino Beam,''
  Phys.\ Rev.\ Lett.\  {\bf 107 } (2011)  041801.
  [arXiv:1106.2822 [hep-ex]].

\bibitem{mutau}
T.~Fukuyama and H.~Nishiura,
  %``Mass matrix of Majorana neutrinos,''
  hep-ph/9702253;
  %%CITATION = HEP-PH/9702253;%%
E.~Ma and M.~Raidal,
  %``Neutrino mass, muon anomalous magnetic moment, and lepton flavor nonconservation,''
  Phys.\ Rev.\ Lett.\ \ {\bf 87} (2001) 011802
   [Erratum-ibid.\ \ {\bf 87} (2001) 159901]
  [hep-ph/0102255];
  %%CITATION = PRLTA,87,011802;%%
C.~S.~Lam,
  %``A 2-3 symmetry in neutrino oscillations,''
  Phys.\ Lett.\ B\ {\bf 507} (2001) 214
  [hep-ph/0104116].
  %%CITATION = PHLTA,B507,214;%%

\bibitem{HPS}
P.~F.~Harrison, D.~H.~Perkins and W.~G.~Scott,
  %``Tri-bimaximal mixing and the neutrino oscillation data,''
  Phys.\ Lett.\ B {\bf 530} (2002) 167
  [arXiv:hep-ph/0202074];
  %%CITATION = HEP-PH 0202074;%%
P.~F.~Harrison and W.~G.~Scott,
  %``Symmetries and generalisations of tri-bimaximal neutrino mixing,''
  Phys.\ Lett.\ B {\bf 535} (2002) 163
  [arXiv:hep-ph/0203209];
  %%CITATION = HEP-PH 0203209;%%
Z.~z.~Xing,
  %``Nearly tri-bimaximal neutrino mixing and CP violation,''
  Phys.\ Lett.\ B {\bf 533} (2002) 85
  [arXiv:hep-ph/0204049].

\bibitem{GR}
A.~Datta, F.~-S.~Ling and P.~Ramond,
  %``Correlated hierarchy, Dirac masses and large mixing angles,''
  Nucl.\ Phys.\ B\ {\bf 671} (2003) 383
  [hep-ph/0306002];
  %%CITATION = NUPHA,B671,383;%%
Y.~Kajiyama, M.~Raidal and A.~Strumia,
  %``The Golden ratio prediction for the solar neutrino mixing,''
  Phys.\ Rev.\ D\ {\bf 76} (2007) 117301
  [arXiv:0705.4559 [hep-ph]].
  %%CITATION = PHRVA,D76,117301;%%
  
  \bibitem{BMorg}
   V.~D.~Barger, S.~Pakvasa, T.~J.~Weiler and K.~Whisnant,
  %``Bimaximal mixing of three neutrinos,''
  Phys.\ Lett.\ B\ {\bf 437} (1998) 107
  [hep-ph/9806387];
  %%CITATION = PHLTA,B437,107;%%
R.~N.~Mohapatra and S.~Nussinov,
  %``Bimaximal neutrino mixing and neutrino mass matrix,''
  Phys.\ Rev.\ D\ {\bf 60} (1999) 013002
  [hep-ph/9809415];
  %%CITATION = PHRVA,D60,013002;%%
G.~Altarelli and F.~Feruglio,
  %``Models of neutrino masses from oscillations with maximal mixing,''
  JHEP\ {\bf 9811} (1998) 021
  [hep-ph/9809596].
  %%CITATION = JHEPA,9811,021;%%
  
  \bibitem{U2}
  R.~Barbieri and L.~J.~Hall,
  %``A Grand unified supersymmetric theory of flavor,''
  Nuovo Cim.\ A\ {\bf 110} (1997) 1
  [hep-ph/9605224];
  %%CITATION = NUCIA,A110,1;%%
 R.~Barbieri, L.~J.~Hall, S.~Raby and A.~Romanino,
  %``Unified theories with U(2) flavor symmetry,''
  Nucl.\ Phys.\ B\ {\bf 493} (1997) 3
  [hep-ph/9610449];
  %%CITATION = NUPHA,B493,3;%%
R.~Barbieri, L.~J.~Hall and A.~Romanino,
  %``Consequences of a U(2) flavor symmetry,''
  Phys.\ Lett.\ B\ {\bf 401} (1997) 47
  [hep-ph/9702315].
  %%CITATION = PHLTA,B401,47;%%
  
  \bibitem{SO3}
S.~F.~King,
  %``Predicting neutrino parameters from SO(3) family symmetry and quark-lepton unification,''
  JHEP\ {\bf 0508} (2005) 105
  [hep-ph/0506297].
  %%CITATION = JHEPA,0508,105;%%
    
  \bibitem{SU3}
  S.~F.~King and G.~G.~Ross,
  %``Fermion masses and mixing angles from SU(3) family symmetry,''
  Phys.\ Lett.\ B\ {\bf 520} (2001) 243
  [hep-ph/0108112];
  %%CITATION = PHLTA,B520,243;%%
  %S.~F.~King and G.~G.~Ross,
  %``Fermion masses and mixing angles from SU(3) family symmetry and unification,''
  Phys.\ Lett.\ B\ {\bf 574} (2003) 239
  [hep-ph/0307190].
  %%CITATION = PHLTA,B574,239;%%
  
  \bibitem{SU3disc}
I.~de Medeiros Varzielas, S.~F.~King and G.~G.~Ross,
  %``Tri-bimaximal neutrino mixing from discrete subgroups of SU(3) and SO(3) family symmetry,''
  Phys.\ Lett.\ B\ {\bf 644} (2007) 153
  [hep-ph/0512313];
  %%CITATION = PHLTA,B644,153;%%
S.~F.~King and M.~Malinsky,
  %``A(4) family symmetry and quark-lepton unification,''
  Phys.\ Lett.\ B\ {\bf 645} (2007) 351
  [hep-ph/0610250].
  %%CITATION = PHLTA,B645,351;%%

\bibitem{AF2}
       G.~Altarelli and F.~Feruglio,
  %``Tri-Bimaximal Neutrino Mixing, A4 and the Modular Symmetry,''
  Nucl.\ Phys.\  B {\bf 741} (2006) 215
  [arXiv:hep-ph/0512103].
   %%CITATION = NUPHA,B741,215;%%
   
      \bibitem{FHLM07}
F.~Feruglio, C.~Hagedorn, Y.~Lin and L.~Merlo,
  %``Tri-bimaximal Neutrino Mixing and Quark Masses from a Discrete Flavour
  %Symmetry,''
  Nucl.\ Phys.\  B {\bf 775} (2007) 120
  [Erratum-ibid.\  {\bf 836} (2010) 127]
  [arXiv:hep-ph/0702194].
  %%CITATION = NUPHA,B775,120;%%

\bibitem{Lam0708}
  C.~S.~Lam,
  %``Symmetry of Lepton Mixing,''
  Phys.\ Lett.\  B {\bf 656} (2007) 193
  [arXiv:0708.3665 [hep-ph]];
  %%CITATION = PHLTA,B656,193;%%
 % C.~S.~Lam,
  %``Determining Horizontal Symmetry from Neutrino Mixing,''
  Phys.\ Rev.\ Lett.\  {\bf 101} (2008) 121602
  [arXiv:0804.2622 [hep-ph]];
  %%CITATION = PRLTA,101,121602;%%
  %C.~S.~Lam,
  %``The Unique Horizontal Symmetry of Leptons,''
  Phys.\ Rev.\  D {\bf 78} (2008) 073015
  [arXiv:0809.1185 [hep-ph]].
  %%CITATION = PHRVA,D78,073015;%%

\bibitem{CHMS1}
C.~Hagedorn and M.~Serone,
  %``Leptons in Holographic Composite Higgs Models with Non-Abelian Discrete Symmetries,''
  JHEP\ {\bf 1110} (2011) 083
  [arXiv:1106.4021 [hep-ph]].
  %%CITATION = JHEPA,1110,083;%%

\bibitem{Lin09}
Y.~Lin,
  %``Tri-bimaximal Neutrino Mixing from A(4) and theta(13) ~ theta(C),''
  Nucl.\ Phys.\ B\ {\bf 824} (2010) 95
  [arXiv:0905.3534 [hep-ph]].
  %%CITATION = NUPHA,B824,95;%%

\bibitem{S4BM}
G.~Altarelli, F.~Feruglio and L.~Merlo,
  %``Revisiting Bimaximal Neutrino Mixing in a Model with S(4) Discrete Symmetry,''
  JHEP\ {\bf 0905} (2009) 020
  [arXiv:0903.1940 [hep-ph]].
  %%CITATION = JHEPA,0905,020;%%

\bibitem{BHL07}
   A.~Blum, C.~Hagedorn and M.~Lindner,
  %``Fermion Masses and Mixings from Dihedral Flavor Symmetries with Preserved
  %Subgroups,''
  Phys.\ Rev.\  D {\bf 77} (2008) 076004
  [arXiv:0709.3450 [hep-ph]].
  %%CITATION = PHRVA,D77,076004;%%

\bibitem{myD4}
A.~Adulpravitchai, A.~Blum and C.~Hagedorn,
  %``A Supersymmetric D4 Model for mu-tau Symmetry,''
  JHEP\ {\bf 0903} (2009) 046
  [arXiv:0812.3799 [hep-ph]];
  %%CITATION = JHEPA,0903,046;%%
C.~Hagedorn and R.~Ziegler,
  %``$\mu-\tau$ Symmetry and Charged Lepton Mass Hierarchy in a Supersymmetric $D_4$ Model,''
  Phys.\ Rev.\ D\ {\bf 82} (2010) 053011
  [arXiv:1007.1888 [hep-ph]].
  %%CITATION = PHRVA,D82,053011;%%

\bibitem{BH09}
  A.~Blum and C.~Hagedorn,
  %``The Cabibbo Angle in a Supersymmetric D14 Model,''
  Nucl.\ Phys.\  B {\bf 821} (2009) 327
  [arXiv:0902.4885 [hep-ph]].
  %%CITATION = NUPHA,B821,327;%%

\bibitem{HMD14}
C.~Hagedorn and D.~Meloni,
in preparation.

\end{thebibliography}



==> Author/boucenna.tex <==
%\def\321{SU(3) $\otimes$ SU(2) $\otimes$ U(1)}
%\def\gsim{\raise0.3ex\hbox{$\;>$\kern-0.75em\raise-1.1ex\hbox{$\sim\;$}}}
%\def\lsim{\raise0.3ex\hbox{$\;<$\kern-0.75em\raise-1.1ex\hbox{$\sim\;$}}}

\begin{center}
{\bf Abstract}\\
\end{center}

  We investigate a model in which Dark Matter is stabilized by means
  of a $Z_2$ parity that results from the same non-abelian discrete
  flavor symmetry which accounts for the observed pattern of neutrino
  mixing.
%
  In this $A_4$ example the standard model is extended by three extra
  Higgs doublets and the $Z_2$ parity emerges as a remnant of the
  spontaneous breaking of the flavor group electroweak symmetry breaking.
%
  We perform an analysis of the parameter space of the model
  consistent with electroweak precision tests, collider searches and
  perturbativity and cosmology. We present detection prospects in direct and
  indirect Dark Matter search experiments.



\vskip5.mm
\section{Introduction}

The existence of Dark Matter (DM) is by now well established, owing
to various cosmological and astrophysical observations. The nature of this non-baryonic
component of the total mass of the Universe is still elusive though, despite great
experimental and theoretical efforts over many years. Elucidating the nature of DM constitutes
one of the most important challenges modern cosmology and particle physics are facing.

However, despite the non-identification of the DM particle (or particles), we do have
some clues about how it \textit{should} be \cite{Bertone:2004pz,Taoso:2007qk}.
Among the most important conditions a DM candidate is required to satisfy are
neutrality, stability over cosmological time scales, and agreement
with the observed relic density.
While the neutrality of the particle is usually easy to accomodate theoretically,
its stability is assumed {\it ad-hoc} in most cases.

A new mechanism of stabilizing DM has been proposed in,Ref.~\cite{Hirsch:2010ru} in which
the stability originates from the flavor structure of the standard model, linking DM to neutrino physics.
Indeed the same discrete flavor symmetry that explains neutrino
mixing patterns~\cite{Schwetz:2008er} is the origin of the DM candidate stability 
\footnote{For models based on non-Abelian discrete symmetries but with a
  decaying dark matter candidate we refer the reader to Ref.\cite{Kajiyama:2010sb} for instance.}.
This link between two sectors that show a striking need for physics beyond the standard model
is attractive and has come under further scrutiny in a series of works, see \cite{Eby:2011qa,Adulpravitchai:2011ei}
for instance.



% The model proposed in Ref.~\cite{Hirsch:2010ru} is based on an $A_4$
% symmetry extending the Higgs sector of the SM with three scalar
% doublets. After electroweak symmetry breaking two of the scalars of
% the model acquire vacuum expectation values (vev) which spontaneously
% break $A_4$ leaving a residual $Z_2$.  The lightest $Z_2$ neutral odd
% scalar is then automatically stable and will be our DM candidate.
% 
% On the other hand, the fermionic sector is extended by four right handed 
% neutrinos which are singlets of \321. Light neutrino masses are generated via a
% type I see-saw
% mechanism~\cite{Minkowski:1977sc,gell-mann:1980vs,yanagida:1979,mohapatra:1980ia,schechter:1980gr},
% obey an inverted hierarchy with $m_{\nu3}=0$ and vanishing reactor
% neutrino angle \footnote{For a similar realisation see~\cite{Meloni:2010sk}.}.
% For pioneer studies on the use of $A_4$ for neutrino physics see
% \cite{Babu:2002dz}.


\section{The Model}
\label{model}
  The model considered in~\cite{Hirsch:2010ru} is based on the $A_4$ discrete group,
the group of even permutations of four objects. Matter fields are assigned to its irreducible
representations in the following way: The standard model Higgs doublet $H$ is assigned to the
singlet representation, while the three additional Higgs doublets
$\eta=(\eta_1,\eta_2,\eta_3)$ transform as an $A_4$ triplet, namely
$\eta\sim 3$. The model has in total four Higgs doublets, implying the
existence of four CP even neutral scalars, three physical
pseudoscalars, and three physical charged scalar bosons.
In the fermion sector we have four right-handed neutrinos; three
transforming as an $A_4$ triplet $N_T=(N_1,N_2,N_3)$, and one singlet
$N_4$.  Quarks are assigned trivially as $A_4$ singlets, as a result
of which there are no predictions on their mixing matrix, as it is
difficult to reconcile quarks with the neutrino sector.

The lepton and Higgs assignments are summarized in table\,\ref{tab1}.
\begin{table}[h!]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c||c|c|}
\hline
&$\,L_e\,$&$\,L_{\mu}\,$&$\,L_{\tau}\,$&$\,\,l_{e}^c\,\,$&$\,\,l_{{\mu}}^c\,\,$&$\,\,l_{{\tau}}^c\,\,$&$N_{T}\,$&$\,N_4\,$&$\,\hat{H}\,$&$\,\eta\,$\\
\hline
$SU(2)$&2&2&2&1&1&1&1&1&2&2\\
\hline
$A_4$ &$1$ &$1^\prime$&$1^{\prime \prime}$&$1$&$1^{\prime \prime}$&$1^\prime$&$3$ &$1$ &$1$&$3$\\
%\hline
%$Z_2$&$-$&$+$&$+$&$-$&$+$&$+$&$-$&$+$&$+$&$+$\\
\hline
\end{tabular}\caption{Summary of the relevant quantum numbers}\label{tab1}
\end{center}
\end{table}

The resulting leptonic Yukawa Lagrangian is:
\begin{eqnarray}\label{lag}
\mathcal{L}&=&y_e L_el_{_e}^c \hat{H}+y_\mu L_\mu l_{_\mu}^c \hat{H}+y_\tau L_\tau l_{_\tau}^c \hat{H}+\nonumber\\
&&+y_1^\nu L_e(N_T\eta)_{1}+y_2^\nu L_\mu(N_T\eta)_{1''}+y_3^\nu L_\tau(N_T\eta)_{1'}+\nonumber\\
&&+y_4^\nu L_e N_4 \hat{H}+ M_1 N_TN_T+M_2 N_4N_4+\mbox{h.c.}
\end{eqnarray}
This way the field $\hat{H}$ is responsible for quark and charged
lepton masses, the latter automatically diagonal.  The scalar
potential is:
%\begin{equation}
%\begin{array}{lll}
\begin{eqnarray}\label{potential}
V&=&\mu_\eta^2\eta^\dagger\eta+\mu_{\hat{H}}^2 \hat{H}^\dagger \hat{H} 
+\lambda_1 [\hat{H}^\dagger \hat{H}]_1^2+\lambda_2 [\eta^\dagger\eta]_1^2
+\lambda_3 [\eta^\dagger\eta]_{1^\prime}[\eta^\dagger\eta]_{1^{{\prime}{\prime}}}\nonumber \\
&+&\lambda_4 [\eta^\dagger\eta^\dagger]_{1^\prime}[\eta\eta]_{1^{\prime\prime}}
+\lambda_{4^\prime}[\eta^\dagger\eta^\dagger]_{1^{\prime\prime}}[\eta\eta]_{1^\prime}
+\lambda_5[\eta^\dagger\eta^\dagger]_{1}[\eta\eta]_{1}
+\lambda_6([\eta^\dagger \eta]_{3_{1}}[\eta^\dagger \eta]_{3_{1}}+h.c.)\nonumber \\
&+&\lambda_7 [\eta^\dagger \eta]_{3_{1}}[\eta^\dagger \eta]_{3_{2}} 
+\lambda_8 [\eta^\dagger \eta^\dagger]_{3_{1}}[\eta \eta]_{3_{2}} 
+\lambda_9 [\eta^\dagger \eta]_{1^\prime}[\hat{H}^\dagger \hat{H}] 
+\lambda_{10}[\eta^\dagger \hat{H}]_{3_1}[\hat{H}^\dagger \eta]_{3_1} \nonumber\\
&+&\lambda_{11}([\eta^\dagger\eta^\dagger]_{1}\hat{H} \hat{H}+h.c.) 
+\lambda_{12}([\eta^\dagger\eta^\dagger]_{3_{1}}[\eta \hat{H}]_{3_1}+h.c.) 
+\lambda_{13}([\eta^\dagger\eta^\dagger]_{3_{2}}[\eta \hat{H}]]_{3_1}+h.c.) 
+\lambda_{14}([\eta^\dagger \eta]_{3_{1}}\eta^\dagger \hat{H}+h.c.) \nonumber\\
&+&\lambda_{15}([\eta^\dagger \eta]_{3_{2}}\eta^\dagger \hat{H}+h.c.) 
\end{eqnarray}
%\label{potential}
%\end{array}
%\end{equation}
where $[...]_{3_{1,2}}$ is the product of two triplets contracted into
one of the two triplet representations of $A_4$, and $[...]_{1,1^\prime,1^\prime\prime}$ is the product
of two triplets contracted into a singlet representation of $A_4$.
%
In what follows we assume, for simplicity, CP conservation so that
all the couplings in the potential are real.
%
For convenience we also assume $\lambda_4 = \lambda_4^\prime$ in order
to have manifest conservation of CP in our chosen
$A_4$ basis.

The minimization of the scalar potential results in :


\begin{equation}
  \vev{ H^0}=v_H\ne 0,~~~~ \vev{ \eta^0_1}=v_\eta \ne 0,~~~~
\vev{ \eta^0_{2,3}}=0\,,\label{vevs}
\end{equation}
where all vevs are real.  This vev alignment breaks the group $A_4$ to
its subgroup $Z_2$ responsible for the stability of the DM as well as
for the neutrino phenomenology~\cite{Hirsch:2010ru}.
%

\begin{center}{\it The stability of the DM}\end{center}

As a consequence of the fields assignments there are no couplings with charged fermions
and quarks. The only Yukawa interactions of the lightest neutral component
of $\eta_{2,3}$ are with the heavy \321 singlet right-handed neutrinos.
This state is charged under the $Z_2$ parity that survives
after the spontaneous breaking of the flavor symmetry.

We now show the origin of such a parity symmetry.  \vskip5.mm

The group $A_4$, has two generators: $S$, and $T$, that satisfy the relations
$S^2=T^3=(ST)^3=I$. In the three dimensional basis $S$ is given by 
\begin{equation}S=\left(
\begin{array}{ccc}
1&0&0\\
0&-1&0\\
0&0&-1\\
\end{array}
\right).\label{z2sim}\end{equation}
$S$ is the generator of the $Z_2$ subgroup of
$A_4$. The alignment $\vev{ \eta} \sim (1,0,0)$ breaks spontaneously $A_4$ to $Z_2$ since $(1,0,0)$ is 
manifestly invariant under the $S$ generator.
The $Z_2$ residual symmetry is defined as
%
\begin{equation}\label{residualZ2}
\begin{array}{lcrlcr}
N_1 &\to& +N_1\,,\quad& \eta_1 &\to& +\eta_1 ,\\  
N_2 &\to& -N_2\,,\quad& \eta_2 &\to& -\eta_2 ,\\
N_3 &\to& -N_3\,,\quad& \eta_3 &\to& -\eta_3 ,
\end{array}
\end{equation}
The rest of the matter fields being $Z_2$ even.
%
The DM candidate of the model corresponds to the lightest $Z_2$-odd
neutral spin zero particle which, for the sake of definiteness, we
take as the CP-even state.
The parameters of the model relevant for the DM phenomenology are 8 (scalar) masses, 7 couplings
  and the ratio of the vacuum expectation values $\tan \beta= v_{H}/v_{\eta}.$

\begin{center}
{\it Neutrino phenomenology}  
\end{center}
We present here the main results  obtained in Ref.\cite{Hirsch:2010ru} concerning the neutrino phenomenology.

The model contains four heavy right-handed neutrinos. It is therefore a special
case, called (3,4), of the general type-I seesaw mechanism~\cite{schechter:1980gr}.  
%
Light neutrinos get Majorana masses by means of the type-I seesaw relation.
The reactor mixing angle $ \theta_{13}$ is null and the hierarchy is inverse.
 The atmospheric angle, the solar angle and the two square mass differences can be fitted.  
The model implies a neutrinoless double beta decay effective mass parameter in the range 0.03 to 0.05~eV at
3~$\sigma$, within reach of upcoming experiments.

Before moving to the calculation of the relic abundance in the next
section we consider the phenomenological constraints on the parameter
space of the model.

\section{Phenomenological constraints}
\label{constraints}

In order to find the viable regions in parameter space where to
perform our study of dark matter, we must impose the following
constraints to the model :

\begin{itemize}
\item {\it Electroweak precision tests} 

  \noindent 
  We compute the effect on $T$ induced by the scalars
  following \cite{Grimus:2007if} and we impose the bounds from
  electroweak measurements \cite{Nakamura:2010zzi}: $-0.08\leq T \leq0.14.$

\item {\it Collider bounds}
%LEP data constrain the scalar sector of the model.

  \noindent 
  The bounds imposed by LEP II on the masses of the neutral scalars in
  our model are similar to those constraining the Inert Doublet Model,
  given in Ref.\cite{Lundstrom:2008ai}.
  The excluded region that we adopt is taken from Fig.7 of
  Ref.\cite{Lundstrom:2008ai}.
  We impose a lower limit on the masses of the $Z_2$ even neutral
  and charged scalars of 114 GeV and 100 GeV respectively. 

\item {\it Perturbativity and vacuum stability}

  \noindent The requirement of perturbativity  imposes the following bounds on the Yukawa couplings of the model
  $\lambda_i \lsim \sqrt{4 \pi}$ and $\tan\beta >0.5$.

Finally we must impose the stability of the vacuum which translate as a set of inequalities to be satisfied by the couplings.
of the models.

\end{itemize}
%


\begin{center}
\begin{figure*}[t]
\includegraphics[width=0.4\textwidth]{Author/dd2.jpg}
\includegraphics[width=0.4\textwidth]{Author/omega.jpg}
  \caption{Left plot: Spin-independent DM scattering cross section 
off-protons as a function of the dark matter mass. The orange regions 
delimited by the dashed (solid) line show the DAMA/LIBRA annual modulation 
regions including (neglecting) the channeling effect~\cite{Fornengo:2010mk}.
%
The green region corresponds to the COGENT data~ \cite{Aalseth:2011wp}.
Dashed and dotted red lines correspond to the upper bound from CDMS
(respectively from \cite{Ahmed:2009zw} and \cite{Ahmed:2010wy}).
XENON100 bounds \cite{Aprile:2011hi} are shown as a solid black line.
%
Right plot: Regions in the plane DM mass ($M_{DM}$) - lightest Higgs boson $M_H$
    allowed by collider constraints and leading to a DM relic abundance
  compatible with WMAP measurements.}
  \label{omega}
\end{figure*}
\end{center}

\section{Relic Density and (In)Direct Detection}
\label{relic}

The thermal relic abundance of $H_2$ is controlled by its annihilation
cross section into SM particles. In order to study the viable regions of the model we
perform a random scan over the 16-dimensional parameter space
($\lambda_i$ and $\tan \beta$ ) and compute the dark matter relic
abundance using the micrOMEGAs package\cite{Belanger:2010gh,Belanger:2008sj} for the points satisfying 
the constraints discussed in Sec.\ref{constraints}. 

In Fig.~\ref{omega} we show the regions with a correct relic abundance
in the plane DM mass ($M_{DM}$) and the lightest Higgs boson mass
$M_{H}$.  For dark matter masses well below the $W^{\pm}$ threshold,
dark matter annihilations into fermions are driven by the s-channel
exchange of the Higgs scalars of the model.

For $M_{H}\lesssim 400$ GeV the annihilation cross-sections are large
enough to obtain the correct relic density for all DM masses up to the
the $W^{\pm}$ threshold. At larger Higgs boson masses, annihilations
into light fermions are suppressed so that the relic abundance is
typically too large unless efficient co-annihilations with the
pseudoscalar $A_2$ are present. 
For lighter dark matter particles, strong co-annihilations cannot be
reconciled with LEPII constraints as these require $M_{A_2}\gsim 100$
GeV \cite{Lundstrom:2008ai}.
%
On the other hand, the absence of points on the strip corresponding to the
line $M_{DM}\sim M_H/2$ is associated to the presence of the $H$
resonance which would enhance the DM annihilation cross section
giving a too small Dark Matter abundance.

For dark matter masses larger than $M_W$ the annihilation cross
section into gauge bosons is typically large enough so that $H_2$ cannot account for
the desired relic density.
%

The prospects for direct dark matter detection in underground experiments are of particular interest.
We see in Fig.\ref{omega} that the model can potentially explain the DAMA annual modulation data
\cite{Bernabei:2010mq,Bernabei:2000qi} as well as the excess recently
found in the COGENT experiment \cite{Aalseth:2011wp}.  The present upper limits on the spin independent
DM scattering cross section off nucleons can already exclude a large region of the parameter space of the model but
do not constrain the mass of the DM candidate. Note that the direct detection plot of Fig.\ref{omega} has
been updated from \cite{Boucenna:2011tj} to include recent results of
XENON100\cite{Aprile:2011hi} and COGENT\cite{Aalseth:2011wp}.


Indirect dark matter searches through astrophysical observations are
not currently probing the model apart from some small regions of the
parameter space where the dark matter annihilation cross section is
enhanced via a Breit-Wigner resonance.
For further details about this study we refer the reader to \cite{Boucenna:2011tj}.


\section{ Conclusions and discussion}
\label{conclusions}

We have studied a model where the stability of the dark matter
particle arises from a flavor symmetry.  The $A_4$ non-abelian
discrete group accounts both for the observed pattern of neutrino
mixing as well as for DM stability.
%
We have analyzed the constraints that follow from electroweak
precision tests, collider searches and perturbativity.
%
Relic dark matter density constraints exclude the region of the
parameter space where simultaneously $M_{DM}\lesssim 40$ GeV and
$M_{H}\gsim 400$ GeV because of the resulting over-abundance of dark
matter.
%
We have also analyzed the prospects for direct  dark
matter detection and found that, although they already exclude
a large region of the parameter space, we cannot constrain the mass of the
DM candidate.
%
In contrast, indirect DM detection is not yet sensitive enough to
probe our predictions.


All of the above relies mainly on the properties of the scalar sector
responsible for the breaking of the gauge and flavour symmetry.
%
A basic idea of our approach is to link the origin of dark matter  to
the origin of neutrino mass and the understanding of the pattern of
neutrino mixing, two of the most oustanding challanges in particle
physics today. Note however that the connection of dark matter to neutrino properties
depends strongly on how the symmetry breaking sector couples to the
leptons.

\section{ Acknowledgments}
This work has been done in collaboration with Martin Hirsch, Stefano Morisi, Eduardo Peinado, Marco Taoso
and Jose W.F. Valle.

\begin{thebibliography}{10}

\bibitem{Bertone:2004pz}
G.~Bertone, D.~Hooper, and J.~Silk, ``{Particle dark matter: Evidence,
  candidates and constraints},'' {\em Phys.Rept.}, vol.~405, pp.~279--390,
  2005.

\bibitem{Taoso:2007qk}
M.~Taoso, G.~Bertone, and A.~Masiero, ``{Dark Matter Candidates: A Ten-Point
  Test},'' {\em JCAP}, vol.~0803, p.~022, 2008.

\bibitem{Hirsch:2010ru}
M.~Hirsch, S.~Morisi, E.~Peinado, and J.~Valle, ``{Discrete dark matter},''
  {\em Phys.Rev.}, vol.~D82, p.~116003, 2010.

\bibitem{Schwetz:2008er}
T.~Schwetz, M.~Tortola, and J.~W. Valle, ``{Three-flavour neutrino oscillation
  update},'' {\em New J.Phys.}, vol.~10, p.~113011, 2008.

\bibitem{Kajiyama:2010sb}
Y.~Kajiyama and H.~Okada, ``{T(13) Flavor Symmetry and Decaying Dark Matter},''
  2010.

\bibitem{Eby:2011qa}
D.~A. Eby and P.~H. Frampton, ``{Dark Matter from Binary Tetrahedral Flavor
  Symmetry},'' 2011.

\bibitem{Adulpravitchai:2011ei}
A.~Adulpravitchai, B.~Batell, and J.~Pradler, ``{Non-Abelian Discrete Dark
  Matter},'' {\em Phys.Lett.}, vol.~B700, pp.~207--216, 2011.

\bibitem{schechter:1980gr}
J.~Schechter and J.~Valle, ``{Neutrino Masses in SU(2) x U(1) Theories},'' {\em
  Phys.Rev.}, vol.~D22, p.~2227, 1980.

\bibitem{Grimus:2007if}
W.~Grimus, L.~Lavoura, O.~Ogreid, and P.~Osland, ``{A Precision constraint on
  multi-Higgs-doublet models},'' {\em J.Phys.G}, vol.~G35, p.~075001, 2008.

\bibitem{Nakamura:2010zzi}
K.~Nakamura {\em et~al.}, ``{Review of particle physics},'' {\em J. Phys.},
  vol.~G37, p.~075021, 2010.

\bibitem{Lundstrom:2008ai}
E.~Lundstrom, M.~Gustafsson, and J.~Edsjo, ``{The Inert Doublet Model and LEP
  II Limits},'' {\em Phys. Rev.}, vol.~D79, p.~035013, 2009.

\bibitem{Fornengo:2010mk}
N.~Fornengo, S.~Scopel, and A.~Bottino, ``{Discussing direct search of dark
  matter particles in the Minimal Supersymmetric extension of the Standard
  Model with light neutralinos},'' {\em Phys.Rev.}, vol.~D83, p.~015001, 2011.

\bibitem{Aalseth:2011wp}
C.~Aalseth, P.~Barbeau, J.~Colaresi, J.~Collar, J.~Diaz~Leon, {\em et~al.},
  ``{Search for an Annual Modulation in a P-type Point Contact Germanium Dark
  Matter Detector},'' {\em Phys.Rev.Lett.}, vol.~107, p.~141301, 2011.

\bibitem{Ahmed:2009zw}
Z.~Ahmed {\em et~al.}, ``{Dark Matter Search Results from the CDMS II
  Experiment},'' {\em Science}, vol.~327, pp.~1619--1621, 2010.

\bibitem{Ahmed:2010wy}
Z.~Ahmed {\em et~al.}, ``{Results from a Low-Energy Analysis of the CDMS II
  Germanium Data},'' {\em Phys.Rev.Lett.}, 2010.

\bibitem{Aprile:2011hi}
E.~Aprile {\em et~al.}, ``{Dark Matter Results from 100 Live Days of XENON100
  Data},'' {\em Phys.Rev.Lett.}, vol.~107, p.~131302, 2011.

\bibitem{Belanger:2010gh}
G.~Belanger, F.~Boudjema, P.~Brun, A.~Pukhov, S.~Rosier-Lees, {\em et~al.},
  ``{Indirect search for dark matter with micrOMEGAs2.4},'' {\em
  Comput.Phys.Commun.}, vol.~182, pp.~842--856, 2011.

\bibitem{Belanger:2008sj}
G.~Belanger, F.~Boudjema, A.~Pukhov, and A.~Semenov, ``{Dark matter direct
  detection rate in a generic model with micrOMEGAs2.1},'' {\em Comput. Phys.
  Commun.}, vol.~180, pp.~747--767, 2009.

\bibitem{Bernabei:2010mq}
R.~Bernabei {\em et~al.}, ``{New results from DAMA/LIBRA},'' {\em Eur. Phys.
  J.}, vol.~C67, pp.~39--49, 2010.

\bibitem{Bernabei:2000qi}
R.~Bernabei {\em et~al.}, ``{Search for WIMP annual modulation signature:
  Results from DAMA / NaI-3 and DAMA / NaI-4 and the global combined
  analysis},'' {\em Phys. Lett.}, vol.~B480, pp.~23--31, 2000.

\bibitem{Boucenna:2011tj}
M.~Boucenna, M.~Hirsch, S.~Morisi, E.~Peinado, M.~Taoso, {\em et~al.},
  ``{Phenomenology of Dark Matter from $A_4$ Flavor Symmetry},'' {\em JHEP},
  vol.~1105, p.~037, 2011.

\end{thebibliography}



